Non-Autoregressive Electron Redistribution Modeling for Reaction Prediction

Reliably predicting the products of chemical reactions presents a fundamental challenge in synthetic chemistry. Existing machine learning approaches typically produce a reaction product by sequentially forming its subparts or intermediate molecules. Such autoregressive methods, however, not only require a pre-defined order for the incremental construction but preclude the use of parallel decoding for efficient computation. To address these issues, we devise a non-autoregressive learning paradigm that predicts reaction in one shot. Leveraging the fact that chemical reactions can be described as a redistribution of electrons in molecules, we formulate a reaction as an arbitrary electron flow and predict it with a novel multi-pointer decoding network. Experiments on the USPTO-MIT dataset show that our approach has established a new state-of-the-art top-1 accuracy and achieves at least 27 times inference speedup over the state-of-the-art methods. Also, our predictions are easier for chemists to interpret owing to predicting the electron flows.

==> Reaction Prediction/0-abstract.tex <==
\begin{abstract}
%Reaction prediction is a fundamental problem in computational chemistry. Existing approaches typically generate a chemical reaction by sampling tokens or graph edits sequentially, conditioning on previously generated outputs. These autoregressive generating methods impose an arbitrary ordering of outputs and prevent parallel decoding during inference. We devise a novel decoder that avoids such sequential generating and predicts the reaction in a Non-Autoregressive manner. Inspired by physical-chemistry insights, we represent edge edits in a molecule graph as electron flows, which can then be predicted in parallel. To capture the uncertainty of reactions, we introduce latent variables to generate multi-modal outputs. Following previous works, we evaluate our model on USPTO-MIT dataset. Our model achieves both an order of magnitude lower inference latency, with state-of-the-art top-1 accuracy and comparable performance on Top-K sampling.

Reliably predicting the products of chemical reactions presents a fundamental challenge in synthetic chemistry. %to drug discovery and  material invention. 
Existing machine learning approaches typically produce a reaction product by sequentially forming its  subparts or intermediate  molecules. Such autoregressive  methods, however,   
%\textcolor{blue}{
not only require a pre-defined order for the incremental construction but preclude
%error propagation along the sequential process  and  
the use of parallel decoding for efficient computation.
%}
To address these issues, we devise a  non-autoregressive  learning paradigm that predicts reaction in one shot. 
Leveraging the fact that chemical reactions can be described as a redistribution of electrons in molecules, we formulate a reaction as an arbitrary electron flow  %\textcolor{brown}{formulation/principle/paradigm? Topology describes the geometric class. Likewise in other sections.}
 and predict it with a novel  multi-pointer decoding  network. %This results in capturing the parallel electron movement, thus the simultaneous  bond making and breaking in  non-mechanistic reactions. %,  where the reaction  diversity  is captured by a latent vector.
Experiments on the USPTO-MIT dataset show that,  our approach has established a new state-of-the-art %Top-1  accuracy   and achieves up to 20 times speed-up for  inference upon the state-of-the-art strategies. tasks show that our method achieves  superior %\textcolor{orange}{(comparable?)}
top-1 accuracy  and  achieves 
  at least 27 times inference speedup  over  the state-of-the-art methods. 
 %\textcolor{orange}{(Mention Interpret-ability?)}
 Also, our predictions are  easier for chemists to interpret owing to predicting the electron flows. % (i.e., mechanism prediction).
\end{abstract}


==> Reaction Prediction/1-introduction.tex <==

\section{Introduction}

% problem formulation, distinguish reaction prediction and product prediction here may be good for a later argument
%    First formalized by~\cite{corey1969computer}, reaction prediction, which aims to identify the probable chemical reactions given the reactants, reagents, and possibly other conditions, has become a fundamental problem in computational chemistry. The ability to predict outcomes of organic reactions allows chemists to analyze the feasibility of chemical reactions and design optimal synthesis routes for target molecules, which is of central importance for synthesis planning and drug discovery. 
 
     Reaction prediction~\cite{corey1969computer}, which aims to predict  the resulting chemical outcomes from  given reactants and reagents, is  a fundamental problem in computational chemistry. Reliably predicting such outcomes %of organic reactions
     enables chemists to analyze the feasibility of chemical reactions and design optimal synthesis routes for target molecules, which is of crucial   importance for synthesis planning, drug discovery, and  material invention. Nevertheless, reaction prediction has remained a foundational challenge owing to the fact that  a typical reaction may involve nearly 100 atoms~\cite{WLN2017jin}, which makes fully exploring all possible transformations  intractable. 
% The background, machine translation models
    %Machine learning based approaches~\citep{struble2020CASP} have achieved great success in reaction prediction, thanks to the large amount of reaction data available. Existing end-to-end approaches either formulate reaction prediction as machine translation~\citep{liu2017retroseq2seq, schwaller2019moltransformer} or graph transformation~\citep{coley2019wldn5, do2019gtpn, sacha2020megan}.     The best-performing methods so far~\citep{schwaller2019moltransformer, sacha2020megan} are autoregressive generative models.     During inference, they generate each output item sequentially, conditioning on previously generated outputs.      For machine translation based models, this inference process often takes hundreds of iterations and incurs high inference latency.     Instead of generating from scratch, several graph-based models~\citep{sacha2020megan} learn to predict a sequence of graph edits. Their output is usually much shorter than the machine translation models, largely reducing inference latency. However, these models cannot achieve state-of-the-art top-1 accuracy and still rely on a specific order and corresponding data augmentation
      \begin{figure}[ht]
        \centering
        %\includegraphics[width = 0.45\textwidth]{figure/preliminary_draft.jpg}
        \includegraphics[width = 0.48\textwidth]{figure/reaction-electron-cropped.pdf}%{electronflow.jpg}
        \caption{%\Jian{too long. make it short}
        Illustration\footnotemark
         of the electron movements %({\em curly arrows}) of pairs of electrons
        in a reaction,  where lines represent single covalent bonds (each comprising 2 shared electrons) and a pair of   dots %around an atom
        representing a lone pair. % (i.e., valence electrons).
        %\CWC{Is this an accurate description? This is not a true mechanitic view since hydrogens are neglected. I would also suggest redrawing this in Chemdraw, if possible, for aesthetics.}
        %\textcolor{brown}{why: Hydrogen is indeed neglected, for the simplicity of our model, as is in other graph-based approaches. Hydrogen can be automatically inferred with valence and electron provided.}
        %\why{
        Each pair of curly arrows show the  movement of one electron pair, %},
        which results in the {\em bond broken} (red curly arrow) and {\em bond formed} (blue curly arrow) in the reaction.        Such electron redistribution yields  the formation and breaking of chemical bonds that change the reactant (left) into product  (right). Our approach here aims to model all the  movements of electron pairs (i.e., curly arrays)  in one shot. %, through simultaneously estimating the changes of electron pairs  between atoms. 
        }
        %\caption{Illustration of an esterification reaction, demonstrating how the transformation of chemical bonds can be represented as parallel flow of electrons. We first represent the reactants as $G^r=(V, E^r)$, where edges $E$ represent pairs of electrons shared between  atoms (i.e.,  nodes $V$). We then model the redistribution of  electrons between atom pairs. Such electron rearrangement thus represents the addition  and removal of  connection bonds in reactants to obtain the product graphs $G^p=(V, E^p)$
        %\Jian{It is very difficult to understand this figure.}\textcolor{blue}{need to visually show how to transform a) into d) with our method's key components included.}
        \label{electronflow}
    \end{figure}
         %(a) and (d) are the reactants and products, respectively. (b)  depicts the electron flows around the center atom. (c) depicts  all the molecule electron flows. Our proposed method aims at capturing the simultaneous flow of electrons in the reactants, thus the non-autoregressive forming of the products. 
         
         \vspace{-2mm}
         
         
         \footnotetext{This  formalism is inspired by, but does not accurately represent, a true arrow pushing mechanism; 
        Hydrogen is  neglected for the simplicity of our model as  that of  other graph-based approaches owing to that  the  Hydrogen can be  inferred with valences and electrons provided.}
    Recently, profound successes have   been achieved by applying machine learning  to cope with the  aforementioned challenge in reaction prediction~\cite{WLN2017jin,struble2020CASP,shi20d}.
    %Some methods  leverage two-stage  learning schemes to decode the reactions~\cite{WLN2017jin,qian2020integrating}. 
    %For example,  \citet{WLN2017jin} propose to first pinpoint the reaction centers and then  utilize the identified  centers to  enumerate candidate reaction products, and  \citet{qian2020integrating} propose to first use  neural networks to estimate the   atom reactivity distribution  and then leverage   rule-based symbolic inference to infer the most probable product molecules. One downside of these approaches is that they  involve multi-stage learning and  cannot be optimized end-to-end. 
    For example, \cite{schwaller2018found,schwaller2019moltransformer} formulate reaction prediction as a problem of sequence translation by representing molecules as  SMILES strings, and Transformer based architecture is used for the translation. More advanced methods~\cite{coley2019wldn5,do2019gtpn,sacha2020megan} represent molecules as graphs and formulate reaction prediction as iterative graph transformation process. 
    %Nevertheless, most  state-of-the-art strategies   leverage gradient descent optimization to embrace an  end-to-end learning paradigm, and   formulate  reaction prediction as a machine translation~\cite{liu2017retroseq2seq,schwaller2019moltransformer} or iterative molecule graph transformation process~\cite{coley2019wldn5,do2019gtpn,sacha2020megan}.  
    Generally, these methods  generate subparts or intermediate molecules of a reaction product in a sequential fashion, through leveraging  successive decoding   steps. %\CWC{WLDN isn't autoregressive or iterative, but does require an enumeration step. The Qian et al. paper mentioned below is also not autoregressive AFAIK} 
    %\textcolor{brown}{why: Other methods usually introduce combinatorial optimization in the decoding process, which involve more computational complexity and cannot be learned end-to-end. \citep{WLN2017jin} requires a enumeration step to generate candidate molecule graphs for ranking, and \citep{qian2020integrating} employs linear programming to regularize the set of potential bonds with chemical heuristics to reach global consistency. }
    %, which  could  take up to  hundreds of iterations. % and thus incurs high inference latency. Also, one such  failed step could invalidate the entire synthesis outcomes. %}  
  %       The latter reduces the number of decoding iterations needed  through integrating structure  knowledge about reactions into the learning. \textcolor{blue}{For example, Sacha et al.~\cite{sacha2020megan}  propose to predict a sequence of graph edits for  forming reactions. Nevertheless, their method still follows an autoregressive editing process  and also requires data augmentation for the graph edits to enhance the training to achieve competitive predictive accuracy. }  \Jian{I do not quite follow this sentence.}

 
         Despite their dramatic  successes,  these  state-of-the-art end-to-end  methods have a major shortcoming, thus hindering their wider applications. That is, these  strategies embrace  an autoregressive decoding procedure, which produces  reaction subparts or intermediate molecule graphs  sequentially, each conditioning on previously generated ones. 
         %\textcolor{blue}{
         Although autoregressive models can model the dependency between the sequential subparts,  there is no unambiguous  principle way of  linearizing  the sequence of steps for constructing a molecular  graph, and one   failed step in such successive  procedure could invalidate the entire synthesis outcomes. %Also, 
         %learning the order for the incremental construction involves discrete, indifferentiable decisions which is a  challenge task for gradient based  models. 
         %Consequently,  these  methods  may   suffer from  error propagation along the
         Furthermore, 
         such iterative generations  hinder   parallel decoding for efficient computation. %, which %. The former can dramatically degrade the model's  predictive accuracy and the latter 
         %prevents  the models from scaling  to  large datasets. \CWC{``Prevents'' is a strong phrase here when Transformers have been applied to datasets that are orders of magnitude larger than reaction datasets ever will be}
         %} \Jian{The first point on error propagation could be risky as I actually think autoregressive models model the dependency between the atoms. I think it would be better to check some literature of non-autoregressive models in machine translation to see their arguments in moving from autoregressive models to non-autoregressive models.} \textcolor{blue}{HG: good point; will check...}

    % our model
%    We propose a novel model for reaction prediction that predicts its outputs in parallel, namely the Non-autoregressive Electron Flow Generator (NEFG).     Inspired by physical-chemistry insights, we recognize an edge in a molecule graph as a pair of shared electrons, and bond transformations as electron flows, which can be predicted in parallel.     Our formulation of electron flow generalizes that of ~\citep{bradshaw2018electro}, by allowing arbitrary, non-linear electron flows and parallel transformation.    In this way, NEFG is capable of predicting chemical reactions in an end-to-end manner without additional data augmentation.



    To cope with the aforementioned  limitations, we propose a novel framework for reaction prediction, which predicts reaction outcomes  in one shot. 
    We leverage the fact that chemical reactions can be described as a redistribution of electrons in molecules. As illustrated in Figure~\ref{electronflow}, such electron movement results in the formation and breaking of chemical bonds that convert the reactants into product molecules~\cite{articleherge}. We here aim to model the \emph{simultaneous}  electron flows in reactants, as such 
    predicting the reaction product is  a byproduct of capturing the  electron rearrangement in the reactants. 
        In a nutshell, we first formulate an edge in a molecular graph as a pair of shared electrons (i.e., a covalent bond) and bond transformations as electron flows. We then propose a novel electron flow principle  
        %generalize the modeling of linear and sequential electron flow, as introduced in~\cite{bradshaw2018electro},
        to describe arbitrary and parallel electron flows in molecules. We further  implement this principle based on the conditional variational autoencoder framework~\cite{SohnLY15} with a novel 
         multi-pointer decoding network to model the incoming and outgoing electron movement probabilities for each atom.  This results in   modeling   arbitrary,  non-linear electron flows and  simultaneous graph transformations for reaction prediction, hence forming reaction products in one shot. Also, our method   possesses beneficial  interpretability through showing how  the reactants react via the reactivities of electrons.
         %As a result, our approach is able to predict chemical reactions in a non-autoregesssive fashion. %end-to-end manner without additional data augmentation.
    We refer to this model as Non-autoregressive Electron Redistribution Framework (NERF).   

% experiments
    %We evaluate our model on the USPTO benchmark dataset.     Our model achieves an order of magnitude higher inference speed and excellent top-1 accuracy, compared to state-of-the-art methods. Enhanced with latent variables, our model can generate diverse multi-modal outputs, with top-k accuracy comparable to autoregressive baselines.
    
    We evaluate our model using  the benchmarking USPTO-MIT dataset.  Our empirical studies show that 
    our approach has established  a new state-of-the-art top-1 accuracy. Moreover, our method achieves    at least 27  times faster for inference  over the state-of-the-art approaches. 
     Our experiments also indicate that the  latent variables introduced in our method enable the generation of  diverse multi-modal outputs, resulting in top-k accuracy comparable to its autoregressive counterparts.
     We also demonstrate that 
      due to the prediction of   electron flows, %(i.e., mechanism prediction),
      our reaction predictions are   easier for chemists to interpret.
    
 \iffalse
 \Jian{We can potentially remove the following paragraphs if there are not enough space.}
   %Our main contributions can be summarized as follows:
   We summarize our main contributions as follows:
%\begin{itemize} \item We generalize the view of~\citet{bradshaw2018electro} to include non-linear electron flows and devise a novel decoder to generate arbitrary electron flow in parallel. \item  We propose a non-autoregressive model for reaction prediction, which achieves state-of-the-art top-1 accuracy with an order of magnitude faster inference. % perhaps this can be removed \item We enhance our model with latent variables and apply a practical searching algorithm to generate diverse multimodal outcomes. \end{itemize}

\begin{itemize}
\item We propose a novel strategy to model simultaneous, non-linear  electron flows in reactants, resulting in generating reaction products in one shot. 
\item  We empirically show that our proposed non-autoregressive  model has established  new state-of-the-art top-1 accuracy on the  USPTO data sets, with  up to 20 times speed-up for inference upon the state-of-the-art strategies.  
\item We  experimentally  show that the  latent variable approach is capable of modeling the  diversity of multi-modal reaction outcomes.
\end{itemize}
\fi



==> Reaction Prediction/2-related_work.tex <==
\begin{figure*}[t]
        \centering
        %\includegraphics[width = 1.0\linewidth]{figure/model_draft.jpg}
       % \includegraphics[width = 1.0\linewidth]{decoding.png}
        \includegraphics[width = 1\linewidth]{figure/model_revision-cropped.pdf}
        %model_final.pdf
       % \caption{Product outcomes  generated by  NEFG. The electron flow on the reactants is predicted via a conditional variational encoder-decoder framework.         }
       \caption{Framework of NERF. The left-bottom depicts the parallel edges in our graph representation $G^{r}$. Encoder  is on the left: the node embeddings are generated by a conditional variational auto-encoder CVAE~\cite{SohnLY15}. Decoder is on the right: the node embeddings   leverage a set of directional PointerNets~\cite{vinyals15pointer} to use attention weights to estimate  the flow of electron pairs between all the atom pairs in the reaction simultaneously. These electron flows thus reflect the changes of edges and then can   be converted  into the addition and removal of edges in the reactant molecule to form the  product molecule $G^{p}$ (right). }
        \label{framework}
\end{figure*}	

\section{Related Work}

%old:(template-free approach)

%learning on SMILES:
%molecule transformer

%learning on graphs:
%wldn
%electro
%gtpn

%new:(graph based)
%GROVER  transformer-based encoder for pre-training
%PGNN    position aware graph encoding
%MEGAN   unified graph transformation for reactions
%GIN     structure aware gnn
%\textbf{Template-based Approach}
Data-driven reaction prediction approaches have historically relied on reaction templates, which define sub-graph matching rules for  similar organic reactions. 
Products are generated by first mapping  reactants to a set of  templates and then applying the pre-defined transformations   encoded in the selected  templates~\cite{ segler2017modelling,segler2017neural,wei2016neural}, optionally followed by a re-ranking step \cite{coley2017prediction}.
%For example,  \citet{coley2017prediction, segler2017modelling,segler2017neural} used heuristic algorithms to extract a large set of reaction templates from the database and introduced neural networks to select the major product by ranking the generated candidates. 
%\citet{wei2016neural} first learned a neural model to classify reactions into different types, based on which they selected templates for the given reactants.
Despite their successful application to synthesis planning, these methods suffer from poor generalization on unseen molecular structures owing to the use of rigidly-defined templates to describe how different chemical substructures may react. % and can not scale well to large data set as they require expensive graph isomorphism. 
%Unlike these methods, our approach is template-free. %, excluding the construction an d maintenance of reaction templates. 


To overcome the limitation of template-based approaches, 
%\citet{kayala2011reaction} first proposed to bypass reaction templates by predicting a series of elementary mechanism steps for reactions. %Nevertheless, this method still requires a rule-based expert system to generate mechanism-level supervision. 
various %data-driven
template-free methods~\cite{WLN2017jin,kayala2011reaction,bradshaw2018electro,WLN2017jin,coley2019wldn5,schwaller2018found,schwaller2019moltransformer,qian2020integrating} have recently been introduced. %For example, 
%\citet{kayala2011reaction}  proposed to bypass reaction templates by predicting a series of elementary mechanism steps for reactions. 
%inspired by  recent advance in neural machine translation~\cite{bahdanau2014nmt,vaswani2017transformer}, 
For example,  %\citet{WLN2017jin} and propose to first pinpoint the reaction centers and then  utilize the identified  centers to      enumerate candidate reaction products, and \citet{qian2020integrating} propose to first use  neural networks to estimate the   atom reactivity distribution  and then leverage   rule-based symbolic inference to infer the most probable product molecules.
two-stage learning methods have been introduced to achieve promising results~\cite{WLN2017jin,qian2020integrating}. 
One downside of these approaches is that they   involve multi-stage learning and  cannot be optimized end-to-end.  
To this end, most state-of-the-art strategies typically embrace an end-to-end,  template-free  learning paradigm. For example,  
\citet{schwaller2018found,schwaller2019moltransformer}  leverage  a sequence-to-sequence framework 
to translate  SMILES~\cite{weininger1988smiles} representations of reactant graphs to those  of product graphs. 
 %They employed a Transformer or long short-term memory (LSTM) architecture to translate canonical SMILES~\cite{weininger1988smiles} representation of reactant graphs to that  of product graphs. 
%However, such methods require learning complex syntactic and semantic rules of SMILES representation and also lack interpretability w.r.t. their predictions. 
%Building upon Weisfeiler-Lehman Networks (WLN),  \citet{WLN2017jin}  proposed a two-stage framework for reaction prediction.  They first trained a WLN to estimate the reactivity score of each atom pair in reactant graphs. Then they employed a separate network to rank all chemically-valid candidates. However, this learning scheme is not end-to-end and also requires extra label annotation. 
\cite{bradshaw2018electro,do2019gtpn, sacha2020megan} formulated reaction prediction as a sequence of graph transformations on  molecule graph. %, where the supervised order of modification is decided by either random sample or heuristic search.
Such autoregressive methods, however, not only require a pre-defined order for the incremental construction but also hinder parallel decoding for efficient computation. 
Our strategy overcomes these challenges by embracing a non-autoregressive  learning paradigm  to generate reaction products in one shot, enabling end-to-end training with parallel decoding for efficient computation.  
%\CWC{Missing https://chemrxiv.org/articles/preprint/Integrating\_Deep\_Neural\_Networks\_and\_Symbolic\_Inference\_for\_Organic\_Reactivity\_Prediction/11659563/1 as related work}8 \textcolor{brown}{why:added in template-free methods}

%Non-autoregressive generation methods bypass the sequential generation  in autoregressive models. Several such strategies have been introduced for molecule generation, including MolGAN~\cite{decao2018molgan}, GraphVAE~\cite{abs-1802-03480} and their variants~\cite{Kwon2019}.
%.  For example,  \citet{gu2018nonautoregressive} proposed non-autoregressive sequence generation for machine translation, in order to parallelize the inference process for better performance on modern hardware accelerators.
 \iffalse
Instead of conditioning each token on previous generated outputs, these approaches factorize the learning objective under the conditional independence assumption:
\begin{equation}
\log p(y \vert x) = \sum^{\vert y\vert} _{i=1} \log p(y_i\vert  x)
\end{equation}
where $y_{i}$ denotes the target token.
Various techniques are introduced to model the dependence between $y_i$ and generate multimodal outcomes. 
Since then various improved methods~\cite{kaiser2018fast,shu2019latentvariable,lee2020iterative} for non-autoregressive machine translation have been introduced. \fi
%\citet{kaiser2018fast} enhanced the model with discrete latent variables.
%\citet{shu2019latentvariable} introduced continuous latent variable with delta posteriors via an EM-like approximate inference algorithm.
%\citet{lee2020iterative} proposed to optimize the translated sentence by iterative refinement in the latent space.
%Instead of providing each token with a corresponding latent variable, we employ a global shared approximated posterior for overall graph nodes.
%Non-autoregressive models for molecule generations have also been proposed, including MolGAN~\cite{decao2018molgan}, GraphVAE~\cite{abs-1802-03480} and its improved version~\cite{Kwon2019}.
%These approaches leverage GAN or VAE to generate bond and atom matrices to form molecule graphs. Nevertheless, they aim at molecule generation from scratch and adapting them to reaction prediction--where the task is closer to revising reactant structures--is not trivial. Furthermore, unlike these methods which aim at predicting molecule graphs, our approach aims to predict a  pseudo-mechanism prediction directly. That is, our method approximates how the reactants react, namely the movement of electrons, as such the reaction products (or the molecule graphs) as just a byproduct of modeling the electron reactivities. As a result,  our method possessed intuitive  interpretability. %For example, if the reaction failed, our model can highlight what electron flows went wrong. 
%Predicting electron flows also has better generation due to the fact that 
%2) unseen reactions also follow an rearrangement of electrons. 
%\CWC{I changed this to ``pseudo''-mechanism, because these are unequivocally \emph{not} real mechanisms.}



To the best of our knowledge, our approach is the first attempt to  modeling electron flows for non-autoregressive chemical reaction prediction. 
The only work we are aware of on predicting molecule electron flow  is  ~\cite{bradshaw2018electro}. 
 Nevertheless, their approach is limited to a subclass of chemical reactions with  ``linear'' electron flows in an autoregressive format. %Also, their method  produces reaction products by predicting a sequence of  linear electron flows that follow  a certain  electron path. 
  In contrast, our strategy predicts electron redistribution in one shot. It embraces  an arbitrary electron flow principle to capture the parallel electron movement, thus the simultaneous bond making and breaking, in reactant molecules.
%\HB{Should we add a sentence explaining: non-autoregressive methods achieves lower accuracy than autoregressive ones in machine translation, but our model achieves comparable or superior results to the state-of-the-art methods. We hypothesize that this is because molecules, unlike sentences, does not have a natural linear order, and therefore our parallel method may be a more natural model. Or should we mention at least non-autoregressive generation as a related work?} 

%\textcolor{brown}{why: Primarily, the we use implicit regularization of electrons for non-autoregressive generation to help reconstruction dependency between atoms. Furthermore, as we discussed in 4.4, the chemical process can be viewed as a parallel process in principle from chemist perspective, which is more consistent with the inductive bias of our model than others.}

==> Reaction Prediction/2.5-preliminaries.tex <==
%\section{Related Work}

% should be rewritten


\section{The Non-Autoregressive Electron  Redistribution  Framework} 
%\CWC{Is this an alternate name? I like it}
In this paper, we formulate the chemical reaction prediction task as a simultaneous  electron redistribution problem. We solve this problem by predicting electron flows around each atom in parallel  with a conditional variational autoencoder.  
Specifically,
we first employ a graph neural network to encode the reactant graphs, where multiple covalent bonds  between  atom pairs are represented by parallel binary  edges --each  depicts two electrons that are shared between the atom pair. In the decoder, the goal is to model the incoming and outgoing electron movement probabilities for each atom (i.e., graph node) in the reactants. Finally, the electron reactivities of the reactants are converted into the addition  and removal of edges in the reactant graphs, forming the reaction products. The proposed framework is depicted in Figure~\ref{framework}, and will be discussed in detail next. 

\vspace{-2mm}

%\section{Preliminaries}
\subsection{Notation and Problem Formulation}
\label{notations}
%In this section, we introduce our notations that build the connection between concepts in chemistry and graph theory, especially the equivalence of electron flow and edge transformation.

% this section builds the mapping between chemistry and graph theory, such that the model section can be free of chemistry terminology
% molecule as a graph
% chemical reactions
% notations, e_ij, f_i
% edges as shared electrons, reaction as electron flow
% edge num in decoder, edge weight in GNN



\iffalse
\textbf{PointerNet and  Transformer}
\textcolor{red}
{
PointerNet was introduced in~\cite{vinyals15pointer} basing on the attention mechanism in sequence-to-sequence model~\cite{}. 
   Instead of using attention to blend hidden units of an encoder to a context
vector at each decoder step, PointerNet  uses  attention weights  as pointers to pointing back to  the inputs. Give a set of nodes $u$, the PointerNet can compute the attention weights between a given node $v \in u$ and all the nodes in $u$:
\begin{equation}
    \text{PointerNet}(v) = \text{softmax}((W^{Q}_{v}) (W^{K} u)^T)
\end{equation}
where %$H \in \mathbb{R}^{L\times k}$ is the index matrix,  $H=[h_1,...,h_L]$, and
$W^Q, W^K \in \mathbb{R}^{k\times k}$ the trainable weight matrices. In typical Pointer Networks, the pointer denotes the action with maximum likelihood/attention in policy, while our pointer refers to the whole attention weights as policy vectors.\\
Transformer was introduced in~\citep{vaswani2017transformer} and relies on attention for  encoding and decoding through weighting average.
\begin{equation}
    \begin{aligned}
     &\text{Attention}(Q,K,V) = \text{softmax}(\frac{QK^T}{\sqrt{d_k}})V\\
     &\text{Multihead}(Q,K,V) = \text{Concat}(\text{head}_1,...,\text{head}_h)W^O\\
     &\text{head}_i = \text{Attention}(QW^Q_i,KW^K_i,VW^V_i)
    \end{aligned}
\end{equation}
where $Q,K,V \in \mathbb{R}^{L\times k}$ are query, key and value input respectively, and $W^Q,W^K,W^V \in \mathbb{R}^{k\times k}$ are trainable weight matrices. \\
Transformer-Encoder(),\\
Transformer-Decoder()
}
\fi

\noindent\textbf{Molecule Graph with Parallel Edges}
%In this paper, an organic molecule (or molecules, if the graph has multiple connected components) is represented as an undirected graph $G = (V, E, \bm{f})$, where $V$ and $E$ are the set of atoms and bonds respectively. Each node $v_i \in V$ is associated with a fix-length feature vector $\bm{f_i}$, each dimension of which corresponds to a property of an atom, e.g., atom type and formal electric charge. Unlike previous works~\citep{sacha2020megan} that typically represent bond type as an edge feature or edge type, we treat different bonds as various parallel edges, which is coherent with our view of bonds as shared electrons between atoms.By $e_{ij} \geq 0$ we denote the number of edges between node $v_i$ and $v_j$, i.e. the number of electrons provided by atom $i$ shared with atom $j$. We allow self-loops in $G$ and let $e_{ii}>0$ denote valence electrons that are not shared with other atoms.
%In this paper, 
We represent 
%\why{
a set of organic molecules 
%} %(or molecules in cases of  multiple connected components)
as  an undirected graph $G = (V, E, f)$, where $V$ and $E$ denote the set of heavy atoms (excluding hydrogen) and bonds, respectively. 
  Each node $v_i \in V$ is associated with a fixed-length feature vector ${f_i}$, each dimension of which corresponds to a certain property of the atom $v_i$ such as atom type or formal electric charge. 
 Unlike previous work where different bond orders are represented by one edge with different features or labels,  
%\textcolor{red}{
our method  treats different bonds as multiple {\em parallel binary edges}, e.g., a double bond is represented as two parallel binary edges  (see far left of  Figure~\ref{framework}).  %} %\Jian{Can we add a figure to illustrate this? I think it is a very important concept. }
%\CWC{A chemist reviewer will ask how this applies to aromatic bonds, which are typically described as bond order 1.5. Pre-emptively addressing how this formalism would extend to that case could be good.}
%\textcolor{red}{why: we formulate the aromatic property as a kind of node feature (and aroma can be reversely indicated via neighbor matching), in addition to the single bond, and for simplicity we omit the prediction of this feature in our model. If necessary, we should add the computing of this prediction.}
%\textcolor{purple}{hb:node features in input: element, segment, reactant indicator, aroma and charge. In output: aroma and charge. We may include more information such as chirality and the number of neutrons in an isotope for more complicated datasets} 



\noindent\textbf{Chemical Reaction as Electron Redistribution}
In this paper, a chemical reaction is described as  a pair of molecular graphs 
$(G^{r}, G^{p})$, where $G^{r} = (V, E^r, f^r)$ is the set of 
%\why{any number of}
reactants and $G^{p} = (V, E^{p}, f^{p})$  the products we aim to predict. 
Note that, these two share the same set of nodes $V$. 
%\noindent\textbf{Chemical Reaction as Electron Redistribution}
%\textcolor{red}{
%Following~\cite{bradshaw2018electro}, 
%A chemical reaction is defined as  a pair of molecular graphs $(R, P)$, where $R = (V, E^r, \bm{f}^r)$ is the set of reactants and $P = (V, E^p, \bm{f}^p)$  the products we aim to predict. Note that, these two share the same set of nodes $V$. \\
%}
From the chemistry perspective, chemical reactions can be defined as a redistribution of electrons in  molecules~\cite{ci00017a011}. In other words, the forming of $E^{p}$  can be described as the rearrangement of electrons in $E^{r}$, which  reflects the addition or removal of edges in $E^{r}$ and hence the forming of the products $E^{p}$. %Aim at  capturing  such electron redistribution, we introduce an arbitrary electron flow topology, which will be discussed next. 



\noindent \textbf{Edge  Change  as Electron Flow in Molecule} 
From a chemistry perspective, each covalent single bond in organic (carbon-based) molecules  represents two electrons that are shared between the atom pair that the bond connects. See illustration in  Figure~\ref{electronflow}. In this paper, we denote $e_{ij}$ ($\geq 0 $ and $  \in E$) as the number of binary edges (i.e., shared electron pairs)  between nodes $v_i$ and $v_j$, ($v_i \in V,  v_j \in V$), i.e. the number of electrons of atom $i$ that are shared with atom $j$. To this end, we allow self-loops in $G$ and let $e_{ii}$ denote the number of %{\color{blue} electrons in}
{\em lone pairs} in atom $i$  (illustrated as a    dot pair around an atom in Figure~\ref{electronflow}), namely valence electrons that are not shared with other atoms. %\Jian{$e_{ii} $ should be twice as the number of lone pairs?} 
%\textbf{Edge Formed and Broken through Electron Flow}
%\label{flowtopology}
%Our approach here aims to model the electron redistribution while transforming reactants $E^r$ to products $E^p$. To attain this goal, we leverage deep neural networks to approximate the incoming and outgoing electron flows for each nodes in the reactants  $E^r$. Doing so, we can estimate the electron rearrangement between any node pair, and thus the change of its edge number. 

From this perspective,  an edge change in a molecule is caused by a valence electron's reactivity. It can form a new bond by sharing with another atom (or form a lone pair through coupling with a sibling atom of its own), or  break an existing bond by withdrawing the sharing.  Also, based on  a chemical rule of thumb known as the Octet Rule, 
valence electrons that are active in reactions and form bonds is typically no larger than 8. This motivates our aim of 
 modeling the incoming and outgoing electron movement probabilities of each of the 8 valence electrons in each atom during reaction. Consequently,  such electron flows  reflect the change of edge number before and after the reaction for each  atom pair ($i$, $j$),  ($v_{i}, v_{j} \in V$), namely
\begin{equation}
\label{deltae}
    \Delta e_{ij} = e_{ij}^p - e_{ij}^r.  
\end{equation} 
%To this end, we learn $\Delta e_{ij}$ by approximating all the edge changes that connect to atom  $i$, denoted as  $\Delta e_{i*}$. Here, * denotes all the nodes that connect to $v_{i}$ in the reactant molecule. 
In other words, through capturing the reactivity probabilities of the  8 valence electrons in each atom,  we can  approximating $\Delta e_{ij}$ directly. By doing this, our method can simultaneously access all the edge changes in the reactant molecule, thus produce the reaction products in one shot. Such   non-autoreggressive nature 
  distinguishes our strategy from previous work in ~\cite{bradshaw2018electro},  which can only handle 
  a subclass of chemical reactions that have  linear electron flows only. %Also, their method  produces reaction products by predicting a sequence of  linear electron flows that follow  a certain  electron path. 

%\noindent\textbf{Chemical Reaction} Formally, a chemical reaction is a pair of molecular graphs defined on the same set of vertices $(R, P)$, where $R = (V, E^r, \bm{f}^r)$ is the reactant and $P = (V, E^p, \bm{f}^p)$ is the product.\\%, $f(\cdot)$ is a function that map each vertex to a fix-length feature vector.
%Let \begin{equation}    \Delta e_{ij} = e_{ij}^p - e_{ij}^r \end{equation} The change in edges from $E^r$ to $E^p$ is precisely captured by the redistribution of electrons $\Delta e_{i*}$ around each atom $i$. $\Delta e_{i*}$ satisfies several chemistry constraints that we incorporate as implicit regularization in designing our decoder. For each node i, we have 
%\begin{equation}
%\label{constraint}
%\Sigma_j \Delta e_{ij} = 0,\quad %\Sigma_j |\Delta e_{ij}| < 2D
%\end{equation}
%The first equation indicates conservation of electrons, and the second indicates the fact that the number of valence electrons is bounded by a small number, and typically most bonds are unchanged by the reaction.As a generalization of the implementation of electron flow proposed by~\citep{bradshaw2018electro}, our formulation $\Delta e_{ij}$ includes arbitrary electron flow topology, instead of just linear electron flows (Figure \ref{decoder}). Moreover, it can be predicted in parallel, allowing non-autoregressive generation. 

%\noindent\textbf{Chemical Reaction}



%\subsection{Modeling Electron Redistribution in Reactants}
%\subsection{Arbitrary Electron Flow Topology}

% is formulated  as a sequence of atoms and is therefore restricted to linear electron flows with certain direction. , we formulate electron flow as electron distribution around each atom, and thus can deal with arbitrary electron flow topology of multiple atoms through the modeling of the electron changes, namely  $\Delta e_{i*}$. 
%As illustrated in  Figure \ref{decoder}, our method can model the parallel  electron flows of atoms, thus enabling the  non-autoregressive generation for reaction prediction. %, which will be discussed  in detail next. 
 
 
 
\if 0
%This change in fact can be  captured by the redistribution of electrons  between  atom $i$ and other related atoms (denoted as $\Delta e_{i*}$) through 
\textbf{Constraints of Chemistry} 
To effectively and simultaneously estimate the aforementioned $\Delta e_{ij}$  in $E^{r}$, we leverage   the following two properties that constrains  chemical reactions. %: \textcolor{red}{{\em Ionization Reluctance}} and {\em \textcolor{red}{Octet} Rule}~\cite{citations here.}. %\Jian{Can we add some citations for the two rules?} 
%following  domain knowledge in chemistry. Typical chemical reactions satisfy two .
%The former states that
First, atoms are seldom ionized and therefore %the number of valence
%electrons  belonging to an atom can be considered  constant  (note: $i$ and $j$ can be the same to indicate the lone pair of electron): 
the number of adding edges and the number of removing edges associated to a specific atom should be equal 
%can be considered  constant 
(note: $i$ and $j$ can be the same to indicate the lone pairs of electrons):
\begin{equation}
\label{constraint1}
\Sigma_j \Delta e_{ij} = 0. 
\end{equation}
%and the latter constraint indicates that
Second, the number of valence electrons, i.e., electrons that are active in reactions and form bonds, is typically no larger than 8 (a chemical rule of thumb known as the Octet Rule). 
Combining with the first constraint, the Octet Rule here suggests that both  the addition and the removal of edges for a specific atom is bounded by 4, namely the summation of the number of  adding edges and the number of removing edges bounded as follows:   % Why "Voctet"? And is this an empirical observation based on the dataset? Not the same as the Octet rule 
\begin{equation}
\label{constraint2}
\quad \Sigma_j |\Delta e_{ij}| < 2D, 
\end{equation}
where $D \in \mathbb{R}$ and represents a small number. %,  as suggested by the Octet Rule. 
\textcolor{red}{HG: For example, in the USPTO-MIT dataset, over 99\% of the atoms have less than 8 valence electrons.}

These two chemistry constraints in fact suggest that 
one can model each atom's electrons activities (i.e., incoming and outgoing electron flows) owing to the fact that there is only a very small number of such electrons for each atom. We attain this goal by deploying an encoder-decoder networks. We will discuss our networks in detail next. 
\fi

%With these chemistry constraints, we next discuss  our encoder-decoder networks for the simultaneous learning of $\Delta e$ for any atom pair in the molecule graphs in order to capture  the  electron reactivity patterns in reactants. 
\iffalse
\textcolor{blue}{
Formally, the aforementioned two chemistry principles require  , i.e., r satisfy the following two conditions, respectively, for  each graph node $v_{i}$:  
%$\Delta e_{i*}$ satisfies several chemistry constraints that we incorporate as implicit regularization in designing our decoder \textcolor{red}{how so and why? why it benefits our method here? (why: the following constraints, the reason should be linked to later sections?) (hb: I think this sentence is confusing and suggest an alternative expression: Typical chemical reactions satisfy two properties, first, atoms are seldom ionized and therefore the number of electrons belonging to an atom is a constant (although atoms can share electrons, they seldom lose or gain electrons. even when they do, our approach is still applicable although less justified). Second, the number of valence electrons (electrons that are active in reactions and form bonds) is no larger than 8. ) The two principles can be precisely captured by the following restrictions on $\delta$ e.}.
%For each node $v_{i}$, we have
\begin{equation}
\label{constraint1}
\Sigma_j \Delta e_{ij} = 0,
\end{equation}
\begin{equation}
\label{constraint2}
\quad \Sigma_j |\Delta e_{ij}| < 2D, 
\end{equation}
where $D \in \mathbb{R}$. 
In other words, Equation~\ref{constraint1} 
indicates the conservation of electrons for each atom (i.e., the Constant property), and Equation~\ref{constraint2} reflects the  fact that  the number of valence electrons is bounded by a small number $D$, and typically most bonds are unchanged by the reaction (i.e., the Cap property). }\Jian{I do not understand this part quite well.}
\fi
%The first equation indicates \textcolor{red}{conservation??(why: the number of electrons overall is invariant.)} of electrons, and the second indicates the fact that the number of valence electrons is bounded by a small number, and typically most bonds are unchanged by the reaction\textcolor{red}{ need further explanation and justification for the  above two sentences?(why: is a picture for illustration of typical reaction enough?)}.


%Our proposed method aims at  modeling the redistribution of electrons, i.e., $\Delta e_{i*}$, in molecule, which results in a  non-autoreggressive nature of our method for reaction prediction. In specific, unlike the  electron flow proposed by~\cite{bradshaw2018electro}, where  an electron flow is formulated  as a sequence of atoms and is therefore restricted to linear electron flows with certain direction, we formulate electron flow as electron distribution around each atom, and thus can deal with arbitrary electron flow topology of multiple atoms through the modeling of the electron changes, namely  $\Delta e_{i*}$.  As illustrated in  Figure \ref{decoder}, our method can model the parallel  electron flows of atoms, thus enabling the  non-autoregressive generation for reaction prediction, which will be discussed  in detail next. 


\iffalse
\begin{figure}[t]
        \centering
        \includegraphics[width = 0.6\linewidth]{figure/preliminary_draft.jpg}
        \caption[width = 0.8\linewidth]{Illustration of Our Formulation for Chemical Reaction. (a) is the reactants, (b) is the electron redistribution process, and (c) the products.}
        \label{transformfig:overview}
\end{figure}
\fi

==> Reaction Prediction/3-model.tex <==
%\section{Non-autoregressive Electron Flow Generator}

\subsection{The Conditional Variational AutoEncoder Framework}

\iffalse
\textcolor{red}{
key ideas: \\
1. mapping electron distribution in the reactants to
that in the product by learning four outgoing electron flows and our incoming electron flows for each node. Some heuristic tricks and chemistry constraints are applied to obtain the change of electron flows and thus the number of edges for each node pair. \\
2. have encoder and decoder (encoder-decoder architecture), but not a VAE framework for learning the reactivity patterns. \\
3. assume electron flows in and out an atom to be independent from that of other nodes, and then this over-strict assumption is mitigated through adding a Gaussian noise to the node embedding in encoding and then sampling from the noisy embedding for decoding. A post-processing step is later applied to remove unnecessary nodes.   \\
4. assume that we know which ones are reagent.\\
5. first learn a continuous latent space by encoding the
reactants and reagents molecular graphs and then generate product graph  through decoding from the learned latent space guided by 
the modeling of the electron flows. \begin{equation}
    P(E_{Product}|E_{Reactant1}, E_{Reactant2})
\end{equation}
}

\textcolor{blue}{why: 1. The chemical constraint is that the changed number of electron pairs between an atom pair is limited by a bound $d$ (typically $d=4$), induced by octet rule. The heuristic to match the two pointer between two atoms (to each other) is to conservatively approximate the number of consistent numbers. (+ - : 0, + + : min, - - : max, as is shown in second part of figure 2.)
The CVAE framework is
\begin{equation}
    \begin{aligned}
    \log p(G_p|E_r) = \log\sum_z p(G_p, z|G_r)\\
    \ge \sum_z \log p(E_p, z|E_r) \\
    =E_{z \sim q(z|G_r, G_p)}\log p(E_p|E_r;z)\\
    + E_{z \sim q(z|G_r, G_p)}\log \frac{p(z|E_r)}{q(z|E_r, E_p)}
    \end{aligned}
\end{equation}
Here $E_p = f(E_r + z)$, where $f(\cdot)$ are transformer decoding layers, and we empirically model $\log p(E_p|E_r, z)$ with L2 loss, or alternatively L1 loss (given the sparsity of delta pointer tensors), so it leads to equation 6. We assume prior $p(z|E_r)$ to be standard Gaussian distribution and posterior $q(z|E_r, E_p)$ to be a reparameterized Gaussian.
\\
3. The Gaussian noise is modeled by the latent posterior computed above, and is deterministically add to the final embedding for decoding without sampling. We post-process the molecule graph to identify the largest separate graph as product, give that most products in the dataset is a single molecule. \\
4. The reagent is preprocessed as molecules which atoms don't appeal in the product molecules. In our NEFG, we add a special embedding to the atoms of the reagent part.\\
5. The electron flow in NEFG is equivalent to the gain or loss of electron pairs, indicating the corresponding modification of chemical bonds between any atom pairs. 
}

% architecture overview, computation graph, and information flow
%In this section, we describe the architecture of NEFG. The overall structure is illustrated in Figure~\ref{transformfig:overview}.The encoder module first encodes the reactants $R$ into representation $h^r$, using a bi-level encoder framework consisting of a GCN module and a graph attention network. The variational encoder module then estimates the posterior distribution of latent variable $z$, which is concatenated with $h^r$ to obtain the product representation $h^p$. % Finally, the decoder module takes $h^p$ as the input and predicts the products $P$. The transformation from $R$ to $P$ is predicted by estimating the electron flows around each node. We use two groups of pointer networks to represent the incoming and outgoing electrons respectively, which we call the influx pointers and the outflux pointers.


%The overall structure follows the conditional variational inference framework, where the variational encoder estimates $p(z|R, P)$ and the decoder models $p(P|z, R)$. The inference procedure is deterministic given latent variable $z$, without the need for autoregressive sampling.
\Jian{We should explain the VAE framework here more clearly. }

\textcolor{blue}{To model the electron flows in molecule, our non-autoregressive 
method NEFG is formulated in the framework of variational autoencoders (VAE)~\cite{kingma13vae}. 
We approach this task  by learning an encoder and a decoder to map
between  electron distribution in  reactant graph $R$ and that in the corresponding product graph $P$; see Figure~\ref{transformfig:overview}. 
}

\textcolor{blue}{
In the probabilistic setting
of a VAE,  the  encoder 
estimates a variational posterior $p(z|R)$ and the decoder defines  a generative distribution $p(P|z)$. $z \in \mathbb{R}^{k}$ is the encoded $k$ dimensional latent vector, which is regularized by a  prior distribution $p(z)$. The learning of the model is to  minimize the upper bound on negative
log-likelihood loss:
− log pθ(G)
	 \begin{equation}
	     \mathcal{L}(P', z; R, P) = \text{recon}(P', P) +  \text{KL}[q(z|R,P), p(z|R)] 
	 \end{equation}
.......
}
%Note that, the decoding procedure is deterministic given latent variable $z$, without the need for autoregressive sampling. % In detail, the encoder module first encodes the reactants $R$ into representation $h^r$, using a bi-level encoder framework consisting of a GCN module and a graph attention network. The variational encoder module then estimates the posterior distribution of latent variable $z$, which is concatenated with $h^r$ to obtain the product representation $h^p$. Finally, the decoder module takes $h^p$ as the input and predicts the products $P$.
Under this context, the transformation from reaction $R$ to product $P$ is predicted by estimating the electron flows around each of the nodes in $V$, where we use two groups of pointer networks to represent the incoming and outgoing electrons respectively (denote as  the influx pointers and the outflux pointers, respectively). 
Next, We will discuss each of the key components in detail. 
\fi

%Our encoder-decoder networks follow the conditional variational auto-encoder (CVAE)  framework~\cite{SohnLY15}. 
Our goal is to model the probability of product graphs $G^p$ conditioning on the reactant graphs $G^r$, i.e., $P(G^p|G^r)$. To model the uncertainty of reaction, we introduce a latent variable $z$ and base the whole model on the conditional variational auto-encoder framework~\cite{SohnLY15}. For training, we aim to maximize the log-likelihood of each training example, i.e., $\log P(G^p|G^r)$. In practice, it is usually computational intractable to maximize the likelihood $\log P(G^p|G^r)$, and a common approach is to maximize an evidence-lower bound (ELBO) of the log-likelihood as below:
%In specific, our  model is trained, with gradient, to maximize the conditional log-likelihood $\log p(E^{p}|E^{r})$, 
%where the variational lower bound of the log-likelihood is used as a surrogate objective function with  Kullback-Leibler (KL) divergence measuring the dissimilarity of  two distributions: 
\begin{equation}
\label{cvaeequ}
\begin{aligned}
    \log p(G^p|G^r) \geq {\mathrm{E}}_{q(z|G^p,G^r)} [\log p(G^p|G^r, z)] -\\
    KL(q(z|G^p,G^r)||p(z|G^r)), 
\end{aligned}
\end{equation}
where $q(z|G^p,G^r)$ is an encoder which defines the variational distribution of the true posterior distribution $p(z|G^p,G^r)$, $p(z|G^r)$ is the prior distribution of the latent variable $z$, and $p(G^p|G^r,z)$ is the decoder. To optimize the lower-bound, we can use the reparametrization trick introduced in the variational auto-encoder~\cite{kingma13vae}. Next, we will introduce our encoder and decoder respectively.  

%This bound  is composed of an  encoder 
%$q(z|E^p,E^r)$, a conditional  prior  $p(z|E^r)$, and a decoder  
%$p(E^p|E^r, z)$. 
%The proposed framework is illustrated in Figure~\ref{transformfig:overview}, and will be discussed in detail next. 
%We will discuss how to compute these three terms in detail next. 




%, which consists of two  components: encoding and decoding.  The input graphs $G^{r}$ are first encoded into a latent variable $z$ that  follows a prior distribution, and then the output products $G^{p}$ are then generated conditioned on  latent variable $z$ sampled from the prior distribution. 

%In specific, during  encoding, we first deploy a graph neural network to encode  each  node in the reactant molecular graphs into a continuous  latent vector $h$. Basing on these embeddings, we then  learn a conditional prior $p(z|E^{r})$  to approximate the true posterior $q(z|E^{r},E^{p})$. The latent variable $z$ here is to regularize the learning of these node vectors $h$ so that both the reaction diversity and the coherence of electron flows across all the individual  nodes are captured. The decoding of our method follows a conditional generative process. We first sample $z$ from the conditional prior $p(z|E^{r})$, %namely $z \sim p(z|E^{r}) $, and   then augment the learned embedding of each node  with $z$. The resulting  augmented node embedding $\hat h$ is used to predict  its electron reactivity. Finally,  basing on the estimated  electron redistribution of the reactants, which reflect the addition and removal of edges, we obtain the product molecule by selecting the largest separate graph. 
%The proposed framework is illustrated in Figure~\ref{transformfig:overview}, and will be discussed in detail next. 

\iffalse
\begin{equation}
    \log p(E_p|E_r)\geq {\mathrm{E}}_{q(z|E_p,E_r)}\log p(E_p|E_r, z) \\ +KL(q(z|E_p,E_r)|p(z|E_r))
\end{equation}
\fi



%The overall structure follows the conditional variational inference framework, where the variational encoder estimates $p(z|R, P)$ and the decoder models $p(P|z, R)$. The inference procedure is deterministic given latent variable $z$, without the need for autoregressive sampling.

%In specific, we first aggregate the neighborhood message around each atom via a graph convolutional network. Then a transformer is employed to capture the long-range interactions between local environments. Afterward, the encoded representations are decoded by a pointer network to predict the electron gain and loss between atom pairs, where a latent posterior is employed to tackle multi-modality in Non-Autoregressive generation. As the number of electrons around each atom in this process is bounded, we assume that there is a limit for the number of incoming and outgoing electrons for each atom. Under the conditional independent assumption, we suppose that two atoms form a shared electron pair only if they are predicted to provide an electron to each other.  


%\subsubsection{Encoding of Molecule Graph Nodes:
\subsubsection{Encoder}
%and  Prior: $q(z|Ep,E_r), p(z|E_r)$}
\label{encodingGCN}
%The goal of the encoder is to compute the $KL(q(z|E^p,E^r)||p(z|E^r))$ term in Equation~\ref{cvaeequ}. 
%Inspired by recent works on graph and molecule representation learning\citep{rong2020grover, xu18howpowerful}, we adopt a bi-level GCN+self-attention graph encoder. 
%Typically, a GNN-based network passes messages between contingent nodes in an iterative manner. However, chemical reactions often involve interaction between distant or even unconnected atoms or functional groups. \citet{sacha2020megan} address this problem by introducing a dummy super-node that is connected to all other nodes. By contrast, our encoder consists of a GNN followed by a graph attention network, in which each atom attends to every other node on the graph. 
%Our encoder consists of a GCN and stack of graph attention layers, following the bi-level information extraction framework~\citep{rong2020grover}. The low-level GCN message passing is guided by connectivity, and focus on local structures within its limited reception field, while the high-level graph attention network is guided by content, and may pass messages between distant parts of the graph to identify the global structure. Our encoder can be interpreted as a differentiable integration of the template-based approach, in which the GNN module explores the local neighborhoods of each atom to identify chemically reactive functional groups, and the inner product attention mechanism searches matched functional groups globally to find potential reaction centers. 
%\Jian{Very difficult to understand...} Following the bi-level information extraction framework~\cite{rong2020grover}, our encoder contains  a GCN network with  a  graph attention layer on the top. The message passing on each layer of the GCN network is guided by graph connectivity, focusing on   local structures within its limited reception field, while the information propagation of the graph attention layer is guided by graph content,  aiming at passing messages between distant parts of the graph to model the global structure of the graph. Under the context of reaction prediction, our encoder can be interpreted as a differentiable integration of the template-based approach, in which the GNN module explores the local neighborhoods of each atom to identify chemically reactive functional groups, while the inner product attention mechanism searches matched functional groups globally to find potential reaction centers. 

%Our encoder takes as  input  a molecule graph $G_{r}=(V,E^r, f)$ of the reactants and  reagents, and  adopts a variant of Graph Convolutional Networks (GCN)~\cite{rong2020grover}  with $L$ layers to encode each node into a continuous latent vector, i.e., node embedding, where Sum pooling is deployed to aggregate information from neighboring nodes during message passing. In each feature vector of the nodes there is a segment to indicate whether it belongs to the reactants or reagents. Doing so, the computation for atoms in reagents can be processed the same way as that in reactants afterwards.% as that in ~\cite{xu18howpowerful}. % in each GCN layer. %\textcolor{blue}{need to explain the notation of $m_{v}$ and $h$ here? hb: the message during GNN message pasing, and hidden states}

%\textcolor{red}{In our NEFG, we add a special embedding to the atoms of the reagent part. What do you mean by that?}\textcolor{blue}{why: It's an optional embedding in the transformer embedding layer, which is equivalent to an additional feature in the feature vector $f_i$.}

%Formally, let
%\textbf{Node Embedding} 


As each reactant is represented as a graph, a natural choice is to encode the atoms of the whole reactants with graph neural networks~\cite{schlichtkrull2018rgcn,rong2020grover}, which have been widely studied to learn representations of different kinds of graphs. Let $k$ $\in \mathbb{N}$ be the embedding dimension and $h^{r(l)}_{i} \in \mathbb{R}^{k\times 1}$  the node embeddings of the $i^{th}$ atom  at the $l^{th}$ layer computed by the GCN $(h^{r(0)}_{i} = f_{i})$. 
%\textcolor{blue}{Note: to simplify our description, we here use the node embedding  $h_{i}$ to denote the concatenation of the node embedding  $h_{i}$ and the node feature $f_{i}$. }


At the $l^{th}$ layer, each node $i$ first aggregates the messages from  %different edge types: $h^{r(l-1)}_{i}$ denote the  embedding node $i$ of the $(l-1)^{th}$ layer in the graph $R$. Then, the aggregated feature for a node $i$ on level $l$ during the GCN message passing, denoted as $m_{i}^{l}$, is computed through aggregating
%all the features of 
its  neighboring  nodes, namely $n  \in \mathcal{N}_i$:  %($\mathcal{N}_i$ denotes the set of neighbors of node $v$): %, as follows.
\begin{equation}
    %\bein{aligned}
    m_{i}^{r(l)} = \text {RELU}(W^{(l)} \cdot \text{SUM}\{h_{u}^{r(l-1)} \vert u \in \mathcal{N}_i\}), 
    %\end{aligned}
\end{equation}
where $ W ^{(l)}\in \mathbb{R}^{k\times k}$ is the trainable weight matrix. The aggregated messages are further combined with the node representation itself by simply taking the summation, yielding a new node representation:
\begin{equation}
    h_{i}^{r(l)} = m_{i}^{r(l)} + h_{i}^{r(l-1)}. %\quad l \in \{1, 2,..., L-1\}.
\end{equation}

\iffalse
Next, this resulting aggregated feature is  then combined with the embedding  of the previous layer, forming  the node's current layer representation, as follows.
\begin{equation}
    h_{i}^{r(l)} = m_{i}^{r(l)} + h_{i}^{r(l-1)}%\quad l \in \{1, 2,..., L-1\}.
\end{equation}
\fi
%\textcolor{red}{Next, the interaction among the neighboring nodes is further modeled with a stack of multi-head self-attention layers as that in~\cite{veli17gat}, resulting  in the representation $h^r_v$ for each node $v$. }
%\textcolor{blue}{should we use $u$ instead of $i$, so to consistent with the equation below? hb: yes! the inconsistency is a careless mistake} 
As graph convolutional networks only capture the local dependency between atoms, to further model the long-range dependency between atoms, we further apply a Transformer Encoder~\cite{vaswani2017transformer} on top of the atom representations learned by GCNs, similar to  \cite{rong2020grover}: %Following  \cite{rong2020grover}, we then  employ  a fully connected graph attention, namely the Tranformer-Encoder attention \textcolor{red}{...need better citation here...}, % as detailed in Section~\ref{notations}),
%in which each self-attention head can attend to all node embeddings (denote $h_{*}$) in the graph  instead of just the neighboring nodes. 
%This results in  the final node embedding of the $i^{th}$ atom in the reactants: 
\begin{equation}
h^{r} = \text{Transformer-Encoder}(h^{r(L)}), %\quad l \in \{1, 2,..., L-1\},
\label{seminodeembedding}
\end{equation}
where $h^{r(L)}$ are the atom representations in the final layer of the GCN, and $h^{r}$ are the final atom representations of reactants. Similarly, we encode the product graphs with the same neural encoder, obtaining the atom embeddings $h^{p}$ for each atom in $G^{p}$. 


%\subsubsection{Regularizing  Electron Redistribution with  Conditional Prior}

%    Our learning  so far is mostly on the node level, which can cause   two issues in reaction prediction: modeling reaction diversity and producing valid  products. 

 %   Capturing the reaction diversity and producing valid products are crucial to reaction prediction.    First, we need to enable our networks to model  the diverse distribution of reactions. In practice, given a set of reactants and reagents,  multiple reactions may take place simultaneously, thus yielding different products. Also, the dominant reaction typically varies dramatically with different reaction conditions such as temperature and pressure, which can also result in   different products.  
    %Therefore,  modeling  the diverse distribution of reactions is important for reaction prediction and generation. 
%    Second, our non-autoregressive  decoding (as will be discussed in Section~\ref{decodingsec}),  simultaneously  predicts the electron flows for each atom, assuming the  conditional independence among these predictions.     In this sense, we  need a mechanism to ensure the  coherence, at a graph level, for these predictions.     Otherwise,  local predictions basing on individual atoms tend to predict one deterministic output, and can easily produce invalid or semantically meaningless graph. %, as a mixture of modalities. 
    %This problem is similar to that in the statistic machine translation systems~\citep{gu2018nonautoregressive} while generating a sequence of output tokens for a sentence. 
    
    
   % Fortunately, the above two issues can be effectively addressed by learning a conditional prior to regularize the learning of the individual node embeddings. %To address the aforementioned issues,   we incorporate  a  regularization term  into our loss function to regularize the learning of the encoder-decoder networks.
%    Our regularizer is inspired by the  constraints imposed in the learned coding vector in  the VAE framework~\cite{kingma13vae}. 
%In specific,  we 
%We regularize the learning of the node embedding $h$, as discussed above, through a graph-level latent variable $z, z \in \mathbb{R}^{1\times k}$. In the end, we expect $h$ encode the static status of each atom (i.e.  node) in the reactant graphs, and $z$ capture the electron flow patterns of  all the  atoms at the graph level during the reaction. In other words, we are interested in modeling the  conditional probability of $z$ given the edges of $E^{r}$ and $E^{p}$, namely $q(z|E^{r},E^{p})$, aiming at capturing the atom redistribution between $E^{r}$ and $E^{p}$. This is in fact the true posterior term under the context of the CVAE framework~\cite{SohnLY15}. 


Once we have the representations for the reactant and product graphs $h^r$ and $h^p$, we then  use them to define our variational distribution $q(z|G^p, G^r)$. %\textcolor{yellow} {We apply a cross attention \textcolor{red}{HG. citation?} module on top of the two sequence representations. The cross attention module attends to the two sequences alternatively, which captures the electron redistribution from the reactants to the products. The cross attention module is similar to a transformer decoder, in which $h^r$ is the target sequence, and $h^p$ is the memory sequence \textcolor{red}{HG. is this correct?}} Since it is used as an encoder instead of a sequence decoder, we allow bidirectional attention and do not use a triangular attention mask \textcolor{red}{HG. I don't get this one}. }\Jian{This is too complicated. This is actually very similar to Transformer-Encoder. We can simply say it is a Transformer for now}.
%\textcolor{blue}{
Specifically, we first pass the $h^{r}$ and $h^{p}$ through a Transformer-Decoder  to compute the cross attention between $h^{r}$ and $h^{p}$. This Transformer-Decoder takes $h^{p}$ as the  input sequence of the first decoder layer   and $h^{r}$ as the last output  sequence of the encoder. 
%\why{
Essentially, the atom representations of product graphs $h^p$ are treated as memory, and the atom representations of reactants $h^r$ are treated as queries, which are updated by attending to $h^p$.
%}
After that, a mean pooling is further applied to all the atom representations of the reactants, yielding a global representation $h^z$ of the reaction: 
%We first \textcolor{red}{obtain the sequential atom representations $h^r$ and $h^p$ respectively (HG: not clear to me)}
% By doing this, we obtain a new set of atom representations for both reactant and product graphs. \CWC{New set of atom representations for each? Or that atom representations that reflect both reactants and products?} \textcolor{brown}{why: both I suppose, since the atom mapping is joint. As is in the equation below, we employ the standard transformer decoder architecture in \cite{vaswani2017transformer}, where $h^r$ is the input from encoder, $h^p$ the input from decoder, and $h^z$ the transformer decoder output.}
\begin{equation}
\begin{aligned}
    %q(z|E^{r},E^{p}) =
    h^{z}=\text{MEAN(Transformer-Decoder}(h^r,h^p)). 
    %h^{z}=\text{MEAN(Transformer-Decoder}(h^r,h^p)), 
    %&z = \text{MEAN}(\text{Multihead}(h^c,h^r,h^r))
    \end{aligned}
\end{equation}
%\textcolor{red}{Independent fully connected layer (HG: this is not a MLP)}
%\textcolor{blue}{
Next, a fully connected layer with  ReLU activation
%}
is further applied to $h^z$ to define the mean and variance of the latent variable: 
\begin{equation}
\label{kldiv}
\begin{aligned}
    &\mu  = W_{\mu}\text{ReLU}(h^z)+b_{\mu},\\
    &\text{log}\sigma = W_{\sigma}\text{ReLU}(h^z)+b_{\sigma}.\\
    %\text{MLP}_{\sigma}(h^z)
\end{aligned}
\end{equation}
where $ W_{\mu}, W_{\sigma}\in \mathbb{R}^{k\times k}$ and $b_{\mu}, b_{\sigma} \in \mathbb{R}^{k\times 1}$ are trainable parameters.
Therefore, the variational distribution is defined as $q(z|G^p, G^r)=\text{Normal}(\mu, \sigma)$. For the prior distribution $p(z|G^r)$, we simply assume it is a simple standard  Gaussian distribution, which does not depend on $G^r$. 

\if 0
 In our approach, we assume the  conditional prior $p(z|E^r)$ to be standard Gaussian distribution. 
Then, with $h^r$ and $h^p$, the   $KL(q(z|E^p,E^r)||p(z|E^r))$ 
is computed by first using another   Transformer-Encoder attention to obtain the final hidden representation: 
%as as follows. First, we  compute $z$  by allowing that the node embeddings of reactants attend to that of the ground-truth products through  a multi-head attention as implemented by a Transformer-Decoder (defined in Section~\ref{notations}) and then we average the resulting multihead attentions:
\textcolor{red}{
\begin{equation}
\begin{aligned}
    %q(z|E^{r},E^{p}) =
    h^{z}=\text{Transformer-Encoder}(h^r,  h^p), 
    %&z = \text{MEAN}(\text{Multihead}(h^c,h^r,h^r))
    \end{aligned}
\end{equation}
}
and then   passing the resulting  $h^{z}$  through a dense layer $\text{Dense}(\cdot)$ to obtain the mean $\mu$ and the standard deviation $\sigma$ 
for the  Gaussian distribution to calculate the $KL$ in closed form. That is, we reparameterize the posterior $q(z|E^r, E^p)\sim N(\mu, \sigma)$ as follows: 

\begin{equation}
\begin{aligned}
    &\mu,\sigma = \text{Dense}(h^z)\\
    &z = \mu\cdot \epsilon + \sigma
\end{aligned}
\end{equation}
where $\epsilon \sim \mathcal{N}(0,1)$ is a sampled random variable.
%here $ h^{p}$ is the node embedding of the ground truth  products, as discussed in Section~\ref{encodingGCN}. %via the same encoder with the reactants, and their parameters is independent (can also be shared alternatively).
%Doing so, such cross attention between reactants and true products enables $z$ to embed atom and electron information from both the reactants and products. 
%This is the node embedding that will be used to replace the one in Equation~\ref{noregul} for our encoder-decoder framework. 
\fi
\iffalse
During reaction prediction, we will not have  
the information from $E^{p}$. A typical approach is to  learn a conditional prior $p(z|E^{r})$ to approximate the true posterior 
$q(z|E^{r},E^{p})$. This approximation   can be 
%With this approximation, we then have a conditional generative process. That is, the latent variable $z$ is sampled from the prior  distribution $p(z|E^{r})$ and the data samples are generated by  a  generative distribution  $p(E^{r},E^{p}|z)$ conditioned on $z$. Here $z \sim p(z|E^{r}) $ and $(E^{r},E^{p}) \sim p(E^{r},E^{p}|z)$.  
 attained by   using the  Kullback-Leibler divergence to match the two distributions:
	 	 \begin{equation}
	 	 \label{electronKL}
	 	 \begin{aligned}
 \mathcal{L}_{kl} &= \text{-KL}(q(z|E^{r},E^{p})|| p(z|E^{r})) \\
 &=E_{z \sim q(z|E^{r}, E^{p})}\log \frac{p(z|E^{r})}{q(z|E^{r}, E^{p})}.
 \end{aligned}
	 \end{equation}
	 This KL lost then can be approximated by a variational lower-bound as that in~\cite{SohnLY15}. 
	 	 	 In this paper, we consider a standard Gaussian for the  conditional prior of  the  latent variable $z$,  namely $p(z|E^{r}) \sim N(\mu, \sigma)$. 
	 	 	 
	 Intuitively, this prior states that the edge patterns of the reactants are projected to a continuous coding space $z$, i.e, $p(z|E^{r})$, that  follows Gaussian distribution. 
	 In this way, if this prior matches the true posterior $q(z|E^{r},E^{p})$, then we  can   draw  samples from $z$, and hence each such sample will represent an edge arrangement  in the reactants and products. 
	 	 Doing so, as will be shown in the experiments, our $z$ not only captures the multi-mode reactions, but also constrains the electron flows of atoms to follow the coherence patterns in the ground-truth, thus generating valid reaction products. 
\fi
%\textbf{The Generative Process} 	



\subsubsection{Decoder}
%: $p(E_p|E_r,z)$}
\label{decodingsec}

\if 0
The goal of the decoder is to calculate the $\log p(E^p|E^r, z)$ term in Equation~\ref{cvaeequ}.

Consider the decoder a  deterministic probabilistic function, and a Guassian distribution  form of its predictions $\hat E^p$, then the decoder term can be rewritten as: 
     \begin{equation}
     \label{decoderappoximat}
    \begin{aligned}     
       \log p(E^p|E^r, z)] 
    & \approx 
    \log e^{-|E^p-\hat E^p|^2} \\
    &=
    (E^p-\hat E^p)^2. \\
&=
\sum_{i,j \in V}
\Vert  e^p_{ij} - \hat e^p_{ij}\Vert ^2_{2}.  
    \end{aligned}
\end{equation} 
 Here, $\Vert \Vert_2$ denotes the $L_2$ norm. 
With this rewritten form,  the computation of $\log p(E^p|E^r, z)$ boils down to the calculation of  $\hat e^p_{ij}$ in our model, which is discussed next. 

\fi


Next, we introduce how to decode the product graph $G^p$ based on the latent variable $z$ and the reactant graphs $G^r$, i.e., $p(G^p|G^r, z)$. As introduced previously, since the atoms are exactly the same between $G^r$ and $G^p$, we need to generate the edge difference between the two sets of graphs. We first generate a new set of atom representations for the reactant graphs (denoted as $\hat{h}^r$) by taking the summation of each atom representation $h_i^r$ and the latent variable $z$, followed by a global transformation through a  Transformer encoder layer:  %Transformer
\begin{equation}
\label{sampleH}
\hat h^r_{i} = h^r_{i} + z,
\end{equation}
\begin{equation}
 \hat h^r= \text{Transformer-Encoder}(\hat h^r).
\end{equation}
\if 0
	 In detail, during decoding we first draw a sample  $z$  from the conditional prior $p(z|E^{r})$, and then add it to the node embedding  $h^{r}_{i}$ as calculated by Equation~\ref{seminodeembedding}: 
\begin{equation}
\label{sampleH}
\hat h^r_{i} = h^r_{i} + z.
\end{equation}
     The resulting node embedding  $\hat h^r$  is then passed through a Transformer-Encoder attention:
     $$\hat h^r= \text{Transformer-Encoder}(\hat h^r).$$
\fi
     Next, these embeddings are  then 
     used to  generate the edge numbers $ e_{ij}^{p}$ for each atom pair ($i$, $j$) in the products. Recall from Section~\ref{notations} that, in order to predict the product graphs, we simply need to model each atom's electrons activities. According to the Octet Rule as discussed in ~\ref{notations},  the number of active valence electrons in an atom is typically at most 8, and
%\textcolor{blue}{
the reactivity of each electron  includes either {\em forming} a  new bond or {\em breaking} an existing bond with another atom (including the atom itself).  % (i.e., all of its incoming and outgoing electron flows). 
     %\textcolor{blue}{
     We here attain this goal  by
      modeling the bond formation and breaking   probabilities associating to each electron in   each atom using  a set of PointerNets~\cite{vinyals15pointer}. %, as will be  discussed in detail next. 
      %}
     
   %At each decoder step of  a sequence-to-sequence model, instead of using attention to blend hidden units of an encoder to a context vector, PointerNet   modulates a content-based attention mechanism over its encoder inputs. 
PointerNet is proposed for selecting an item from a set of items using attention mechanism.  In our setting, for each electron of an atom $i$ in reactants $G^r$,   PointerNet can compute the attentions between atom $i$ and all the  atoms  in $G^r$ (including $i$). The attentions are calculated through a softmax function, thus each of those attention weights can be interpreted as a probability. That is, through the attention weights, a PointerNet provides us the   probabilities of atom $i$ initiating an  electron flow  with all the atoms in the graph. %$j$ (or a lone pair in case $i = j$). 
      %^{1 \times k}$. % is the attention weight between the atom pair $(i, j)$. %This $w_{ij}$ here in fact  indicates a probability of an electron flow from atom $i$ to atom $j$.

%According to the Octet Rule as discussed in ~\ref{notations},  the number of active valence electrons in an atom is at most 8 and 
%\textcolor{blue}{
%the reactivity of each can be identified as either {\em forming} a  new bond or {\em breaking} an existing bond.  

Consequently, for each electron $d$,  we deploy two PointNets: one capturing its probability (denoted $w^{+d}$)   of  bond formation and  another the probability (denoted $w^{-d}$) of  bond breaking.  We denote these two types of PointerNet as    {\em BondFormation}  and {\em BondBeaking}  PointerNets, respectively. That is, in total our model has 8  BondFormation  PointerNets and 8  BondBeaking   PointerNets, and all the 16 PointerNets are shared among all the atoms in the reactants. 
 Formally,  
give a set of nodes $\hat h^r$ in the reactants $G^{r}$, a  PointerNet  
can compute an attention weight to reflect the probability of an electron flow   from  atom $i$ to any  atom $j$ in $G^r$:  
        \begin{equation}
w_{ij}^{(+d)} = \text{PointerNet}_d^+( \hat h^r, i, j), d\in{1,2,\cdots, 8}
    \end{equation}
    \begin{equation}
w_{ij}^{(-d)} = \text{PointerNet}_d^-( \hat h^r, i, j), d\in{1,2,\cdots, 8}
    \end{equation}
    
where $w_{ij}^{(+d)}, w_{ij}^{(-d)} \in [0,1]$.
%}
%In addition, according to the Octet Rule as discussed in ~\ref{notations},  the number of active valence electrons in an atom is at most 8. That is, potentially we can have up to 8 incoming or outgoing electron flows for each atom. Therefore, our method here  deploys 8  influx PointerNets in order to model the maximum number of   incoming  electron flows in an atom. Similarly, we deploy  anther 8 outflow PointerNets to monitor all the  possible outgoing  electron flows of an atom. 
%Formally, let D=8. Then  for the $d^{th} $ ($d \in D$) PointerNet, an atom $i$'s  incoming   or outgoing attention weight  for an atom pair ($i, j$)   aims at  estimating the influx or outflow electron flows, respectively, between the atom pair. These two directional attentions are denoted as $w_{ij}^{(d)+}$ and $w_{ij}^{(d)-}$, respectively. 
    

%\textcolor{blue}{
    With the attentions  computed by the 16 PointerNets,  the overall %edge transformation around
    electron reactivity for an atom pair ($i$,  $j$) %each node (Fig~\ref{decoder}(b)) is
    then can be  approximated by  calculating the difference between the summation of  the  8   BondFormation  attentions  and  that of the 8  BondBreaking  attentions: %}%\textcolor{red}{HG: This function could be fine-tuned?}  \CWC{4 v 8 change is confusing without explanation IMO}
%    The difference here aims to  fulfill the {\em Constant Atom Counts} constraint in     Equations~\ref{constraint1}:  %\textcolor{blue}{what is the intuition here for projecting weights to edges? what are the benefits? the intuition is, the weight represents the electron density, and therefore the existence and number of bonds. the benefit is simplicity for I believe using a classifier to predict the existence and number of bonds would be essentially equiavalent in performance}
    \begin{equation}
    \label{ppointer}
        \begin{aligned}
        &\Delta  \tilde w_{ij} = \sum_{d=1}^8 w^{(+d)}_{ij} - \sum_{d=1}^8 w^{(-d)}_{ij}. \\
        \end{aligned}
    \end{equation}
    %\textcolor{blue}{
    Here, the first and second summations represent the additions and the removals of edges, respectively. %}
    \if 0
    It is worth noting that, according to      Equations~\ref{constraint1}, these attentions  should satisfy the following constraint:
        \begin{equation}\sum_{ j \in v} \Delta  \tilde w_{ij}=0.    \end{equation}
        \fi
    %This bound on  the  attentions is important for  the learning of the $\Delta  \tilde w_{ij}$ across all the node pairs in $G^r$ to be stabilized. 
%    \Jian{Not so clear starting from here. Did we do the rounding during the training as well or only use it during inference. If rounding is used in training, how to do backpropagation.} 
 %   \textcolor{brown}{why: No rounding in training, just continuous L-norm loss.}
    Doing so,  $\Delta \tilde w_{ij}$ thus reflects the  change of edge number between the atom pair ($i$, $j$). %, i.e.,  $\Delta e_{ij}$  as defined in Equation~\ref{deltae}. 
%In other words, we here leverage $\Delta \tilde w$ to approximate the density of  $\Delta e$ for any atom pair in $R$. %, thus predicting the existence and the number of bonds, between atom pairs. 
 Next, 
%    After having  $\Delta \tilde w_{ij}$,  %$\Delta e_{ij}$, %inference step is used to sample discrete prediction for edge transformation $\Delta e$ from the  continuous weights $\Delta \tilde w$. In detail, the edges in the product is first estimated by combing the edges in the reactant and the estimated edge modifications:
    we then add it to the  existing number of edges, i.e., $e^r_{ij}$, resulting in  the  new edge number $\hat e_{ij}$ between the atom pair ($i$,$j$): 
    %\textcolor{blue}{inconsistent notation here? otherwise, we need to explain a bit  about the notation here.}: 
    \begin{equation}
    \label{wwij}
        \hat e_{ij} = e^r_{ij} + \Delta \tilde w_{ij}.
    \end{equation}
    
    
    %\textcolor{blue}{
% This predicted $\hat e_{ij}$ thus can be used to %compute the  in turn results in maximizing
%compute the expectation  of $p(G^p|G^r,z)$ using  the following expanded form (assuming conditional independence):  %}
%  follow a  Gaussian distribution, owning to that each of them is generated by a softmax function.  In this sense, the edge number $e_{ij}^p$ in the products can be considered as sampling from the Normal distribution of $\hat e_{ij}$: $$e_{ij}^p \sim \text{Normal}(\hat{e}_{ij}, I).$$
%\textcolor{purple}{hb:The distribution is highly unimodal, therefore rounding the expectation to the closest integer practically yields the maximum likelihood estimation} \textcolor{brown}{why:not necessarily normal, or binomial distribution, etc, just a empirically approximation is sufficient.}
%Consequently,  we then can  aggregate these estimations to form the probability model for our decoder $p(G^p|G^r,z)$. In specific, the generation of product graph $G^{p}$ can be decomposed into the parallel generations of edges, i.e., $e_{ij}^p$. Our approach  here assumes  that  the electron flows between pairs of atoms are independent given the latent variable $z$. Hence, the probability of the generation of the reaction products   can be computed as the products of the generation probabilities of all   edges:
Finally, we define our likelihood function as:
\begin{equation}
\begin{aligned}
   \log p(G^p|G^r,z) &= \sum_{(i,j)\in E^p} \log p(e_{ij}^p|G^r,z)\\
   &\propto -\sum_{(i,j)\in E^p} (e_{ij}^p-\hat{e}_{ij})^2.
    \end{aligned}
\end{equation}
%Following a  common  approach for VAE~\cite{kingma13vae}, we maximize the above log likelihood by  minimizing  an $L_2$ reconstruction loss as follows:
%\begin{equation}
%\begin{aligned}
%    \mathcal{L}_2 & = \sum_{(i,j)\in E^p} (e_{ij}^p-\hat{e}_{ij})^2
 %   \end{aligned}
%\end{equation}
%Combining with the KL Divergence loss as computed through  Equation~\ref{kldiv}, the above reconstruction loss therefore  forms the final loss of our variational auto-encoder networks. We minimize this final loss function  through gradient descent with mini-batch training in order to fulfill 
%our design goal of maximizing the log-likelihood  $\log P(G^p|G^r)$ as described in Equation~\ref{cvaeequ}.    
    
\textbf{Generation} 
%We empirically observe that  the distribution of $\Delta \tilde w_{ij}$ (Equation~\ref{ppointer})  is highly unimodal. Hence, %rounding the $\hat e_{ij}$ computed  in Equation~\ref{wwij} to the closest integer in practically yields the maximum likelihood estimation of $ p(\hat e_{ij}|G^r,z)$. In this sense, 
%to obtain an instance of 
%the molecule graph $G^p$ after training, 
%In practice,
In practice, given a set of reactant graphs $G^r$, to generate the product graphs, $\hat e_{ij}$ is   rounded to the closest integer to obtain  the  edge number between the atom pair, namely $e^p_{ij}$ :  
    \begin{equation}
    \label{edgeGeneration}
        e_{ij}^p = \text{round}(\text{min}(\hat e_{ij}, \hat e_{ji})).
    \end{equation}
Doing so,  we then have the resulting modified  graph $ G^{p}$. 
%Note that, although most reaction products only contains some of the atoms in the reactants. $G^{p}$ contains all atoms in $G^{r}$ and typically consists of multiple molecules. %In this way, we not only predict the labeled main product, but also infer side-products in an without supervision. 
During evaluation, a reaction is correctly predicted if the ground truth product is a subgraph of our prediction $G^{p}$ (more  detailed illustration will be presented in Figure~\ref{explainable} in the Experiment section).

%In practice, we observe that $\Delta \tilde w_{ij}$ is typicall y almost an integer and simply rounding to the closest integer yields the most likely prediction of $\Delta e$. To this end,
%in our approach
%As the last step of our approach, we conduct a post-processing to convert this modified graph into the product molecule graph $G^{p}$.
\subsection{Atom Feature 
%\why{
Construction and
%}
Prediction
}
%\textcolor{blue}{To this end,  ${f_i}$  includes element, segment, reactant indicator, aroma property and charge status. During decoding, our model predicts both the aroma property and charge status besides the electron flows of each atom. In this way, we can generate aromatic bonds  described as bond order 1.5. Note that, our model has the flexibility to extends this vector  ${f_i}$ to include other properties of an atom such as  chirality and the number of neutrons in an isotope for more complicated datasets. 
%}
\if 0
\textcolor{red}{
    \begin{equation}
        L_{norm} = \sum_{(i,j)\in E^p}\Vert\Delta\hat w_{ij} - \Delta w_{ij} \Vert _1
    \end{equation}
    }
  \fi
%\Jian{define the probability function here.}
%\why{
We assign each graph node (i.e., atom) with a unique identifier as its positional embedding~\cite{you2019positionaware}. This ensures that atoms in different chemical environments have distinct node representations.
The input features of atoms include atom type, charge, aromaticity, segment embedding and positional embedding. There is no edge feature in our model.
%}\\

Our proposed NERF framework can  easily  incorporate domain knowledge owing to the fact that each atom has its own embedding $h^{r}$.  %\textcolor{brown}{(should be $\hat h^r$)}.  
In addition to  predicting the edge changes in the reactants, our  model can naturally leverage the atom embedding $h^{r}$ to  predict  an atom's other properties such as its electron charges, aromatic property and chirality.  

To this end, we  pass  the atom  embedding $h^{r}_{i}$ through a MLP layer to generate the predicted probabilities of this atom's aromatic property. 
Such prediction thus can  help us to recover the aromatic bonds, which are typically described as alternating single and double bonds, in the resulting product graphs. %In this scenario, an MLP layer is needed to add to the  NEFG network with 

%$\hat f_{i}^{(j)} $ and then comparing with the one-hot embedding of each of the target features $f_{i}^{(j)}$ through a Entropy loss:
%\textcolor{red}{HG. a set of classifiers here? entropy loss for each node feature prediction (compared to one-hot embedded label.} \textcolor{brown}{yes.}: \textcolor{red}{h + node features (charge status, reactant indicator, aromatic bond, 3D structural info. }
\if 0
\begin{equation}
    \hat f_{i}^{(k)} = \text{Softmax}(W^{(k)}\hat h^r_i+b^{(k)}).
\end{equation}
\begin{equation}
    L_{CE} = \sum_{i,j}\text{Cross-Entropy}(\hat f_{i}^{(j)}, f_{i}^{(j)}).
\end{equation}
\fi
%Such predicted aromatic property will help us to recover aromatic bonds in the products. 

%\textcolor{brown}{why:$ L = L_{recon} + L_{KL} = L_{norm} + L_{CE} + L_{KL}$}

\if 0
\begin{equation}
\begin{aligned}
    p(G^p|G^r,z) &= \prod_{(i,j)\in E^p} p(e_{ij}^p|G^r,z) \cdot \prod_{i\in V^p} p(f_i|G^r,z) \\ 
    &=\prod_{(i,j)\in E^p} \text{Normal}(e_{ij}^p|\hat{e}_{ij}, I)
    \cdot \prod_{i\in V^p} p(f_i|\hat f_i) .
    %\textcolor{red}{HB:Normal??}
    \end{aligned}
\end{equation}
\fi




==> Reaction Prediction/4-experiment.tex <==
\section{Experimental Studies}
    % overall performance, performance on subsets (classified with electron topology), inference speed (over autoregressive models)
    
    % CWC: Consider adding another graph-based approach https://chemrxiv.org/articles/preprint/Integrating_Deep_Neural_Networks_and_Symbolic_Inference_for_Organic_Reactivity_Prediction/11659563/1
    
    \begin{table*}
      \caption{Top-k accuracy on USPTO-MIT; Best results in \textbf{bold}. We also show if the comparison model can be parallelly  trained in an  end-to-end fashion.  %\textcolor{red}{is the $\checkmark$ a ``No'' here?}
      $^\dagger$ indicates that the results were copied from its published paper.
      %\textcolor{brown}{
      The bracket indicates the method's  learning taxonomy: ``combinatorial'' for    parallel optimization,  ``graph'' for  graph translation, and ``sequence''  for an auto-regressive generation. %Our model is graph-based, yet our paradigm bypass the dependency of atoms via non-autoregressive variational framework.%}
      }
      \label{topk}
      \centering
      \begin{tabular}{lllllcc}
        \toprule
        \multicolumn{4}{r}{Accuracies(\%)}  \\
        \cmidrule(r){2-5}
        Model Name(scheme)  & Top-1 & Top-2 & Top-3  & Top-5  & parallel & end-to-end \\
        \midrule
        WLDN$^\dagger$ (combinatorial) & 79.6 & - & 87.7 & 89.2 & $\checkmark$  & $\times$ \\
       % Seq2Seq &80.3 & 84.7& 86.2& 87.5 & $\times$  & $\checkmark$ \\
        GTPN $^{\dagger}$( graph) & 83.2 & - & 86.0 & 86.5  & $\times$  & $\checkmark$ \\
       % WLDN5 &85.6& 90.5& 92.8& 93.4  & $\checkmark$  & $\times$ \\
        Transformer-base $^{\dagger}$ ( sequence)& 88.8  & 92.6 & 93.7 & 94.4 & $\times$   & $\checkmark$ \\
        MEGAN$^{\dagger}$(graph) &89.3& 92.7 &94.4 & \textbf{95.6}  & $\times$  & $\checkmark$ \\
        Transformer-augmented $^{\dagger}$( sequence)& 90.4  & \textbf{93.7} & \textbf{94.6} & 95.3  & $\times$  & $\checkmark$ \\
        Symbolic$^{\dagger}$ (combinatorial) & 90.4 & 93.2 & 94.1 & 95.0 & $\checkmark$ & $\times$\\
        \hline
        %\hline
        NERF  %($\mathcal{L}_{kl}=1$)
        & \bf{90.7$\bf{\pm{0.03}}$} & 92.3$\pm{0.22}$ & 93.3$\pm{0.15}$ & 93.7$\pm{0.17}$ & $\checkmark$  & $\checkmark$ \\
     %   Ours($\mathcal{L}_{kl}=2.5$) & 74.9 & 89.1  & 92.4 & 94.0 & $\checkmark$  & $\checkmark$ \\
        \hline
    %    Ours(ensemble of 2) & 90.7 & 92.7  & 93.8 & 94.7 & $\checkmark$  & $\checkmark$ \\ %        Ours(ensemble of 2) & 90.7 & 92.7  & 93.8 & 94.7 & $\checkmark$  & $\checkmark$ \\ 
        
      %  \bottomrule
        % all are decreased by 0.3%
      \end{tabular}
    \end{table*}    
 %   \vspace{-2mm}
           \begin{table*}[h]
      \caption{%Single Model Accuracy for Different Reaction Topology and
      Computation  speedup  (compared with Transformer) }\label{speed}
      \centering
      \begin{tabular}{llcc}
        \toprule
  %      \multicolumn{5}{r}{Accuracy(\%)}  \\
   %     \cmidrule(r){2-6}
        Model Name  &  Wall-time &Latency & Speedup  %& speedup (Latency) 
        \\ \hline
        Transformer (b=5) & 9min & 448ms &1 $\times$\\% & 1$\times$\\
        MEGAN (b=10) & 31.5min & 144ms & 0.29 $\times$ \\%& 3.1 $\times$\\
        Symbolic &  $>$7h & 1130ms & 0.02 $\times$ \\%& 0.4$\times$\\
        \hline
        NERF & 20s &17ms & 27$\times$\\% & 26$\times$\\     
        % this can be improved with oversampling
        \bottomrule
      \end{tabular}
    \end{table*}
    
\subsection{Experiment Setup}
    \paragraph{Dataset}
    Most of the publicly available reaction datasets are  derived from the patent mining work of Lowe~\cite{Lowe2012ExtractionOC}, where the chemical reactions are described using a text-based representation called SMILES and RDKit library  \cite{landrum16rdkit} is used to transform the SMILES strings into molecule graphs. 
       We evaluate our model using 
       the popular benchmarking USPTO-MIT dataset. %two such  benchmark  datasets: %USPTO-STEREO,
       %USPTO-MIT and USPTO-LEF. %Each set contains less reactions than the former one and is roughly a subset of the former.
    %The  \textbf{USPTO-MIT} 
    This dataset was  created by~\citet{WLN2017jin} by removing duplicate and erroneous reactions from \citet{Lowe2012ExtractionOC}'s original data and filtering to those with contiguous reaction centers. The resulting dataset has about 480K samples and has been  widely used for benchmarking~\cite{schwaller2018found,WLN2017jin,do2019gtpn,bradshaw2018electro,schwaller2019moltransformer}. 
    %\HB{contiguous reaction centers?}
    
    %Following the literature, We use the RDkit library  \cite{landrum16rdkit} to transform SMILES strings into molecule graphs. 
%The \textbf{USPTO-LEF} task is a subset of USPTO-MIT.  ~\citet{bradshaw2018electro} created this subset by selecting only linear reactions. The original subset  is not publicly available, but we recreated it by following the same rules as described in~\cite{bradshaw2018electro}. 
%\item \textbf{USPTO-STEREO} has  about 1M samples. In contrast to  USPTO-MIT and USPTO-LEF,  USPTO-STEREO underwent less filtering and thus most of the stereochemical information was kept. 
        %We evaluate our model using  the benchmark dataset USPTO-MIT, which has been widely used  in previous works~\cite{schwaller2018found,WLN2017jin,do2019gtpn,bradshaw2018electro,schwaller2019moltransformer}. The dataset contains 480k reactions with  10 classes, where reactants, reagents, and products are represented as SMILES strings. Following the literature, We use the RDkit library  \cite{landrum16rdkit} to transform SMILES strings into molecule graphs. 
       
              \textbf{Data Prepossessing} For the USPTO-MIT dataset, we empirically observe that  the change of binary edges does not exceed  4. We, therefore, reduce the number of  PointerNets deployed, as described in Equation~\ref{ppointer}, from 8 to 4. That is, in this implementation, we only use 4 BondFormation and 4 BondBreaking PointerNets. 
              %\why{
              In addition, %Additionally, in practice,
              we observe that although the computational cost is insensitive to the number of PointerNets, increasing the number of PointerNets from 4 to 8 had no accuracy benefit; on the other hand, performance degraded while decreasing the number of PointerNets  below 4.
              %}
              Also, for this dataset, there are 0.3\% of reactions do not satisfy this implementation's settings. Hence, we exclude these reactants from both training and testing, and then just subtract our predictve accuracy on the remaining reactants by  0.3\% as our model's final accuracy.
        %4 of positive pointers and 4 of negative pointers in each atom point to itself, so 8 of 16 pointers are always unused, so we use 4 in/out pointers, instead of maximum 8.
%\textcolor{red}{node features regarding formal charge and aromatic bond are constructed additional to typical ones.} 
    For the node features, we follow literature for the construction. Additionally, we  include the formal charge and aromatic bond property  as part of our atom feature. 
Also, we add an extra atom feature distinguishing   reactant from reagent. We do so by  following the filtering process as in~\citep{schwaller2019moltransformer}. % that identify molecule sub-graphs in the input graph which don't contain any atoms in ground truth products, and split the input into the reactant and reagent parts.

       
       
    \textbf{Model Configuration}
        We implement NERF  using Pytorch \cite{paszke19pytorch}. Both the Transformer-encoder and Transformer-decoder  contain 6 self-attention layers with 8 attention heads as in the original Transformer  configuration. %; 6 GCN layers and 6 self-attention layers each with 8 heads?}\textcolor{blue}{why:The encoder and decoder each have 6 attention layers, and encoder additionally have GCN layers}.
        The node embedding dimension is 256 and the dimension of the latent representation is 64. The model is optimized with AdamW \cite{kingma14adam} optimizer at learning rate $10^{-4}$  with linear warmup and linear learning rate decay. We train the models  for 100 epochs with a batch size of 128 using two Nvidia V100 GPUs (took about 3 days). 
        
 
    \textbf{Evaluation Metrics}
        %Similar to \citep{WLN2017jin}, we use top-k exact match accuracy as our evaluation metric. Following previous works, we choose $k$ from $\{1, 2, 3, 5\}$ in our experiments. 
        Similar to \cite{WLN2017jin}, we use top-k exact  SMILES string match accuracy as our evaluation metric, which is the percentage of reactions that have the ground-truth product in the top-k predicted molecules sets. Following previous works, our experiments choose $k$ from $\{1, 2, 3, 5\}$. 
        
\textbf{Generating Multimodal Outputs}
To draw (approximate) the  top-k samples from our method  efficiently, we sample $m$ latent vectors ($m \geq k$) at increasing temperatures  and take the first $k$ different predictions as an approximation to the top-k predictions. %\Jian{where is T defined?}
Specifically, at temperature $T\in \mathbb{N}$, the latent vector is drawn from $N(\textbf{0}, T*\textbf{I})$. Using a temperature higher than 1 improves sampling efficiency by increasing diversity and therefore reducing duplicate samples. 

We use the $k$ different samples drawn at the lowest temperature for the approximation of the top-k samples since samples drawn at high temperatures tend to be noisier and less credible. 
We find this sampling  works well in practice, and provides a lower bound of the real top-k accuracy.        
        
%   \subsection{Performance on USPTO-MIT}     
        
   % \paragraph{Comparison Baselines}
        %We compare the performance of our model with several previous methods.
        
        \textbf{Comparison Baselines} 
        We evaluate the proposed approach using the following six baselines. 
%\cite{WLN2017jin, bradshaw2018generative, do2019gtpn,schwaller2019moltransformer}
%\begin{itemize}
%\item \textcolor{red}{ELECTRO~\cite{bradshaw2018electro}}
%need to explain why ELECTRO~\cite{bradshaw2018electro} was not used as a baseline. Unlike ours, their method models  a sequence of linear electron flows.  } 
    \begin{itemize}
    \item{\textbf{WLDN}}~\cite{WLN2017jin} is a two-stage approach built upon Weisfeiler-Lehman Network, which first identifies a set of reaction centers,  enumerates all possible bond configurations, and then ranks them. %WLDN5 \cite{coley2019wldn5} is an enhanced version of WLDN model.
   % \item \textbf{Electro} \citet{bradshaw2018generative} captures the reaction mechanism as electron paths to generate the sequence of bond modifications between atoms.
    % \item \textbf{GTPN}~\cite{do2019gtpn} leverages a Graph Policy Network \cite{you2018gcpn} for Reinforcement Learning to model the molecule graph transformation as a Markov Decision Process(MDP). 

 \item{\textbf{GTPN}}~\cite{do2019gtpn} treats a chemical reaction as a sequence of graph transformations and employs reinforcement learning to learn a policy network for such transformations.
 \item{\textbf{Transformer-base}}~\cite{schwaller2019moltransformer} leverages the power of Transformer~\cite{vaswani2017transformer} to predict SMILES strings of product graphs. 
 \item{\textbf{Transformer-augmented}}~\cite{schwaller2019moltransformer} leverages the data augmentation of SMILES strings to boost the performance of Transformer-base.
       % \textcolor{red}{.................}
 \item{\textbf{MEGAN}}~\cite{sacha2020megan} models chemical reactions as a sequence of graph edits, and learns to predict the sequence autoregressively.
\item{\textbf{Symbolic}}~\cite{qian2020integrating} integrates symbolic inference with the help of chemical rules into neural networks.
%\end{itemize}  
        \end{itemize}
%    Note that, among these methods, molecule transformer~\cite{schwaller2019moltransformer} achieves state-of-the-art top-k accuracy for k=1, 2, 3, while MEGAN~\cite{sacha2020megan} is the state-of-the-art approach for k=5, 10.
    %\CWC{Consider adding Qian et al. preprint}
          We here compare with a variety of strategies  including methods deploying  parallel optimization,   graph  translation, and sequential reaction generation, as indicated by the text in the brackets in Table~\ref{topk}. % Our model is graph-based, yet our paradigm bypass the dependency of atoms via non-autoregressive variational framework.
 

\iffalse
    \begin{table*}[h]
      \caption{Single Model Accuracy for Different Reaction Topology and Inference Latency}\label{speed}
      \centering
      \begin{tabular}{llllllcc}
        \toprule
        \multicolumn{5}{r}{Accuracy(\%)}  \\
        \cmidrule(r){2-6}
        Model Name  & non-linear & parallel  & single-linear & wall time &latency &speedup \\
        Transformer (b=5) & 82.1  & 86.8   & 89.8  & 9min & 448ms &1 $\times$\\
        
  %      Transformer (b=1) & -  & -   & - &9min & 416ms &1.06$\times$\\
        ours & 80.6 & 87.2 & 90.4 & 20s & 17ms & 26$\times$\\     
        % this can be improved with oversampling
        \bottomrule
      \end{tabular}
    \end{table*}
    % both the oversampling and the number of beams are hyper parameters... perhaps we should argue the top1 is more important?
\fi

    
        \subsection{Predictive Accuracy}


  
    Table~\ref{topk} presents the predictive accuracy obtained by the testing models  on the USPTO-MIT task.
    %\textcolor{red}{Models were trained and tested with the reactants and reagents separated in the input.} \CWC{How does this work in terms of the model? Do you filter what edge changes are able to be predicted? Do you add an atom-level feature indicating if it's a reagent and not a reactant? I don't think enough details are given.}\textcolor{brown}{why: We add an extra atom feature indicating belonging to reactant/reagent of each atom. We follow the filtering process as \citep{schwaller2019moltransformer} that identify molecule sub-graphs in the input graph which don't contain any atoms in ground truth products, and split the input into the reactant and reagent parts.}
    
    Results in Table~\ref{topk} indicate that,  
       our method outperformed all the comparison baselines in terms of top-1 accuracy, establishing a  new state-of-the-art top-1 accuracy of 90.7\% for the USPTO-MIT task.   
       As can be seen in Table~\ref{topk}, NERF  outperformed Transformer-base and MEGAN by 1.9\% and 1.4\%, respectively. Promisingly, 
   our  approach also outperformed the two-stage  optimization method with logic inference, i.e., Symbolic, and the Transformer-augmented strategy, which leverages data augmentation to boost its accuracy from 88.8\% obtained by its non-augmented version, i.e., Transformer-base. 
   
   %Here, the 
    %Transformer-augmented method augments the train set by choosing 4 different orderings for each reaction to improve its predictive performance of its baseline model, namely Transformer-base. Such gains brought by the data augmentation is owning to the following fact. Autoregressive generation method such as Transformer typically requires an output sequence for supervision, while molecules typically have a non-linear structure without a natural sequential ordering. 
   %This arbitrary ordering may confuse the model from learning the structure of molecules, which can be alleviated by choosing ordering randomly for training  each epoch. This is attained by the Transformer-augmented approach through   augmenting the train set by choosing  different orderings for each reaction~\cite{schwaller2019moltransformer}.
   % On the contrary, since our model decodes in parallel, we do not rely on such data augmentation techniques to achieve superior  accuracy.
    
    
    
    When considering the top-2, top-3 and top-5 accuracy. The NERF 
    performed on par with 
    %the top-k accuracy of NEFG is comparable with
    the state-of-the-art methods, with the worse accuracy on the Top-5 case. % across different $k$ in terms of the top-k accuracy. 
    
    %\why{
    We also conducted a statistical significance testing for Table~\ref{topk}.
   We ran our models with 5 random seeds. Since the variance of baseline models was not available, we conducted One Sample T-test instead of
    Paired T-test against the  Transformer model (SOTA, 90.4\%). Our T-test indicates that our model’s superior top-1 accuracy was
    statistically significant (the p-value was smaller than $10^{-5}$). 
    %}
    %Also, for the top-k accuracy (k with 1,2,3,5), our standard
    %deviations obtained were 0.03\%, 0.22\%, 0.15\%, and 0.17\%,
    %respectively. }
 
%\textcolor{red}{When comparing the parallel approach ... }

    %\textcolor{blue}{
   % It is worth noting that   autoregressive generation typically requires an output sequence for supervision, while molecules typically have a non-linear structure without a natural sequential ordering.    This arbitrary ordering may confuse the model from learning the structure of molecules, which can be alleviated by choosing ordering randomly for training  each epoch.    As shown in Table \ref{topk}, augmenting the train set by choosing 4 different orderings for each reaction is necessary for the Transformer (denoted Transformer-augmented) to achieve competitive  performance~\cite{schwaller2019moltransformer}.    On the contrary, since our model decodes in parallel, we do not rely on such data augmentation techniques to achieve superior  accuracy.
    %Table~\ref{topk} shows the performance of transformer with and without data augmentation

    
%    \textcolor{red}{Transformer-augmented takes advantage of data augmentation which represents a different setting than that of the other comparison methods. }
 %   \CWC{In some ways, yes, but it's a trivial data augmentation strategy}
    

 
 
 
\subsection{Computation Speed-up}
%\Jian{This paragraph is too long....}
         %   \vspace{-2mm}
        
     We evaluate the computational cost of the comparison baselines with two evaluation metrics: Latency and Wall-time. 
          Latency measures 
      time needed to generate the prediction for  a single test sample. %The Latency typically dominates the computation cost for methods that need to  heuristically search the output space to generate the reaction outcomes or       to generate topology of molecule graphs from scratch. %The former includes        MEGAN and Transformer, where  beam search is deployed, and the Symbolic method, where  linear programming is leveraged to conduct global optimization.       The latter includes  Transformer and Symbolic, where graphs are generated iteratively from scratch. 
    The  Wall-time  pictures a more practical evaluation for modern batch-based neural models. It measures the time needed for  all the testing  samples, taking into the fact that  batch-based testing is further affected by data parallelism, e.g.,  GPU  acceleration %(all comparison methods except symbolic benefit from such acceleration),
    and CPU multi-core process. % (both Symbolic and our method benefit from this). 
     
    We compare the Wall-time and Latency for inference with the state-of-the-art machine translation based model Molecular Transformer, graph translation model MEGAN, and rule based model Symbolic. %~\citep{schwaller2019moltransformer}.
    %we split the test set into single-linear, parallel linear, and non-linear according to the reaction electron flow topology~\cite{electron_flow}, and compare the accuracy on each class separately. Figure \ref{topology} illustrates samples from the three subsets.
    %In this experiment, we also split the test set into single-linear, parallel linear, and non-linear according to the reaction electron flow topology~\cite{electron_flow}, and compare the accuracy on each class separately. 
    % add figures for the three cases
    
    %\textcolor{purple}{hb:  
    All models are evaluated on a single Nvidia V100 GPU and a Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz with 28 cores. %(to emphasize that we use the same platform for all models, no matter it is CPU or GPU intensive)%}
 %Both NEFG and Transformer are evaluated on a single Nvidia V100 GPU \textcolor{brown}{as well as ours}, and Symbolic on Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz with 28 multi-cores. The Wall-time here is the total time used for evaluation on the test set of USPTO-MIT.
    %The models are trained and tested with the reaction and reagents mixed, which is more challenging and close to the real application. \CWC{Do you have a different results table showing this quantitative performance?}
    As the  Transformer and MEGAN relies on a beam search to find the most probable prediction, the beam size $b$ is a hyper-parameter that determines the trade off between the accuracy and computational efficiency.
    We show results of  Transformer for $b = 5$, the default setting for top-5 inference, as further increasing $b$ leads to only marginal improvement in accuracy. Likewise, for MEGAN we set $b=10$. 
            %\textcolor{purple}{hb:
            All experiments uses the maximal possible batch size that fits in the GPU memory (32GB).
        % megan batch size = 256 
         We do not include the time spent on loading/saving, preprocessing and postprocessing the data. 
         More specifically, for MEGAN and Transformer, we only count the time spent on beam search. For our model, we count the time spent on computing the forward pass. For Symbolic, we count the time spent on Gurobi sampling. %, which is the major part.%}
         Results are presented in Table~\ref{speed}. 
    
        Table~\ref{speed} indicates that our method achieved  at least 27 times inference speed-up when compared to the comparison  models. For example, the Transformer took 9 minutes for the Wall-time  and MEGAN and Symbolic took over 31 minutes and 7 hours respectively, while  our strategy finished the reaction generations in just 20 seconds. Also, for the Latency, all the three comparison baselines require over 100ms, yet our strategy needs only 17ms. As shown in the last  column of Table~\ref{speed}, our method achieves at least  27 times speedup over the Transformer models in terms of  Wall-time. 
%        \textcolor{brown}{why:Since symbolic is a two-stage method, we test its speed for the second stage of symbolic inference, which cost most time in the algorithm. Moreover, because it cannot make use of batch-wise optimization, instead compute one sample by one, it suffers from the high overall time consuming.  }
        
%Unlike our method which generates the reaction in one shot,  Transformer  heavily depends on autoregressive sampling during inference.     It iteratively samples the output tokens during inference, with the number of iterations equals to the tokenized SMILES sequence length.     By contrast, our model predicts the reaction in a single parallel forward pass, leading to a significant improvement in computation efficiency.     As for the Symbolic, it  is a two-stage method that cannot make use of batch-wise optimization. As a result, it computes one sample by one, thus it suffers from the high overall time consuming.

%        The models are tested on a Single Nvidia V100 GPU (32GB), the wall time and latency doesn't contain the time spent on preprocessing and postprocessing the molecules.
        
 %  \vspace{-2mm}
            \begin{table}[h]
      \caption{ Accuracy (\%) on  individual reaction topology. Best results are in \textbf{bold}. }\label{invididualaccuracy}
      \centering
      \begin{tabular}{lllll}
       \toprule        %\multicolumn{5}{r}{Accuracy(\%)}  \\         \cmidrule(r){2-6}
         & Linear & Branch  & Cyclic \\
        Sample dist. 
        & 73.7\% & 16.9\% & 0.5\%\\
        \hline
        ELECTRO & 87.0 & N/A & N/A\\
        
       % MEGAN & &  & \\  we donnot have a checkpoint for separated setting, to be   - -added in the appendix
        Symbolic&\textbf{92.5}&83.2&68.0\\
        Transformer-base &  89.8 &  80.0 &  66.5\\
        Transformer-augmented&91.4&82.5&\textbf{74.9}\\
  %      Transformer (b=1) & -  & -   & - &9min & 416ms &1.06$\times$\\
  \hline
        NERF & {92.2} & \textbf{85.1}& {71.4} \\     
        % this can be improved with oversampling
        \bottomrule
      \end{tabular}
    \end{table}
 %   \vspace{-2mm}
         \begin{figure}[h]
        \centering
        %\includegraphics[width = 0.8\linewidth]{figure/topology_cropped.pdf}
        \includegraphics[width = 1.0\linewidth]{figure/reaction-topology-revision.pdf}
        % reaction-topology-update-cropped.pdf
        \caption{Different reaction topology (left) and reaction products generated by our method (middle), 
        where the green numbers distinguish different oxide atoms. 
        On the right, the blue lines denote new bonds formed, and the red lines denote  bonds broken.  
        %\why{where the green number is the mark to distinguish two different oxide atoms.{More reaction topology placed here}}
        %\textcolor{red}{add some cases for each category.} 
        %\CWC{Are these auto-generated? Visualization is kind of hard to follow, esp. since only one of the bonds in the double bond is marked yellow for the second example. I would recommend drawing in Chemdraw}
        }  
        \label{topology}
    \end{figure}
    \begin{figure}[h]
        \centering
        %\includegraphics[width = 1.0\linewidth]{figure/model_draft.jpg}
       % \includegraphics[width = 1.0\linewidth]{decoding.png}
        \includegraphics[width = 0.9\linewidth]{figure/topology-expend-revision.pdf}
       % \caption{Product outcomes  generated by  NEFG. The electron flow on the reactants is predicted via a conditional variational encoder-decoder framework.         }
       \caption{Extra examples of our reaction topology. (a)(b)(c)(d)(e) are samples with reaction centers~\cite{WLN2017jin} of linear, branch, cyclic, parallel and multi topology respectively. The red edges are bonds broken while blue edges denote  bonds formed.
       }
        \label{topology+}
\end{figure}
   % \vspace{-2mm}
 
%\vspace{-2mm}
\subsection{Accuracy on Individual Topology}     %  \vspace{-2mm}
In addition to the overall accuracy, we also examined our model's performance on different types of reaction topology. 

  %      In this experiment, we  split the test set into three types of topology identified by the chemists, namely  single-linear, parallel linear, and non-linear according to the reaction electron flow topology~\cite{electron_flow}.
        %\CWC{This doesn't match the topologies shown in the Figure and discussed later -- why not?}
%, and compare the accuracy on each class separately.
        %\textcolor{brown}{why: 
        \citet{electron_flow} considers three types of   reaction topology, namely Linear, Cyclic, Complex for the full USTPO dataset  as an organizing principle for the known reactions. Nevertheless, for the USTPO-MIT dataset, this will result in extremely imbalanced categories with over 99\% of samples falling into the  Linear topology. %, which is challenge to evaluate a model's performance on the minority categories. 
        Inspired by the topology used in~\cite{bradshaw2018electro},  
        we  
         %split the dataset into more detailed segments, and 
         select three types of  representative topology, namely Single-Linear  (%a.k.a. USTPO LEF dataset as used in~\cite{bradshaw2018electro}
          73\% of total samples), Branch (tree-structured, with 17\% of total samples) and Cyclic (cyclic and complex reactions with 0.5\% yet important samples) (illustrated in the left  of Figure~ \ref{topology}). %, and other reactions left is  less than 10\%. % are not representative/critical. 
         %In a word, our taxonomy is somehow a improvement of both ElECTRO and chemists used, which is tailored for the full USTPO dataset, weighting the machine learning methodology and the chemical principles.%}
        
        
                We compare our method with the Transformer (both base and augmented versions), Symbolic, and ELECTRO~\cite{bradshaw2018electro}. 
    %\textcolor{brown}{why: 
    Results in Table~\ref{invididualaccuracy} show that our model achieved superior or performed on par with the four comparison baselines on all the three types of topology. For example, our method achieved the best accuracy on the Linear, Branch, and Cyclic, except obtaining slightly lower accuracy than that of Symbolic on Linear and that of Transformer-augmented on Cyclic. On the other hand, the ELECTRO performed the worst on the Linear topology, while  Symbolic achieved the best on Linear type but lower accuracy on the Branch and Cyclic. Also, although Transformer-augmented obtained the highest accuracy on the Cyclic, but it obtained lower accuracy than our method on the other two categories, namely Linear and Branch. 
These results suggest that our method performs well over all the individual topology types.     
    %reaches excellent performance on the three topology, compared to the best results, and is relatively balanced even without data augmentation(transformer) or ensemble(symbolic).  As for ELECTRO, our models retain the advantage of mechanism interpretation, but can be generalized to complicated topology rather than restricted on single linear (LEF). %}
    

    
\subsection{Topology and Prediction Visualization}
   % \vspace{-2mm}
 Figure~\ref{topology}  visualizes some generated reaction products that follow   the three types of topology as described above. 
The left column of Figure~\ref{topology} depicts the three types of topology, namely Linear, Cyclic, and Branch. The middle two columns show the reaction of transforming reactant on the left to the product on the right, which is correctly predicted by our method. The right  column of the figure presents the corresponding electron flows captured by our model during the reactions, where the blue lines denote new bonds formed and the red lines denote bond broken.  
%\textcolor{red}{Showing Figure~\ref{topology}, each with some real reactions.

%\textcolor{brown}{why: The topology of reaction transformation corresponds to data structure of three styles: list, tree, and cyclic graph, which is both feasible to compute and meaningful in chemical principles, taking extra consideration of data distribution.}
Figure~\ref{topology} indicates that our model can not only predict reactions from various types of topology, but also clearly show the electron flows that result in the final reaction products.

%\why{
In Figure~\ref{topology+}, we also depict additional cases of our model predictions. In addition to the aforementioned three topology, we here also list parallel and multi topology, covering all of our taxonomy. Parallel topology refers to the reactions where there are parallel edges breaking or forming, and Multi are those with multiple reaction centers, each representing a series of bond forming and breaking.
%}
%\vspace{-2mm}



\subsection{Interpretability}    

\citet{bradshaw2018electro} show intuitive interpretability of their model due to the prediction of mechanism. 
Since our model embraces predicting  the pseudo-mechanism, namely the  electron flows during the reactions, our predictions are  also easy for chemists to interpret. %\CWC{Add reference to Bradshaw here since that is a benefit they established?} 


       \begin{figure}[h]
        \centering
        \includegraphics[width = 0.9\linewidth]{figure/interprete-redistribution-cropped.pdf}
        \caption{A reaction  correctly predicted by our model. Our model predicts the direction and the number of electron flows, which are denoted by arrow pushing and real values  respectively. 
        These predictions clearly show what caused the  bond making and breaking during the reaction, thus it is much easier for chemists to interpret.
        %\textcolor{brown}{
        The product in the green box is the ground truth, which is predicted correctly, and we also predicted the  byproducts (in the purple box) at the same time when generating  the whole predicted graph $\hat G^p$.
      %\textcolor{red}{Add cases here...}
        }  
        \label{explainable}
\end{figure}   

\if 0
   % \vspace{-2mm}
\begin{table}[h]
    \centering
      \begin{tabular}{lllll}
        \toprule
        \multicolumn{4}{r}{Accuracies(\%)}  \\
        \cmidrule(r){2-5}
        Model Name    & Top-1 & Top-2 & Top-3  & Top-5\\
        \midrule
        WLDN$^{\dagger}$   & 83.1 & 89.3 & 91.5 & 92.7 \\
        
    %    \CWC{See comment}\\ % I did this evaluation on the LEF test set in my SI:  http://www.rsc.org/suppdata/c8/sc/c8sc04228d/c8sc04228d2.pdf
        Seq2Seq$^{\dagger}$ & 82.6 & 87.3 & 88.8 & 90.1  \\
        ELECTRO$^{\dagger}$ & 87.0 & 92.6 & 94.5 & 95.9  \\
     %   \textcolor{red}{otherbaselines} &&&&\\
        GCN$^{\dagger}$ & 88.3 & 92.9 & 94.2 & 95.3 \\
        Transformer-base $^{\ddagger}$ & 91.1 & 94.3 & 95.1 & 95.7\\
        %Transformer-augmented (not trained)& \\
        MEGAN$^{\ddagger}$  &91.8& 94.7& 96.0& 96.9\\
        \hline
        \hline
        Ours($\mathcal{L}_{kl}=0.4$)  & 91.0& 92.6 & 93.4 & 93.8   \\
        \bottomrule
      \end{tabular}
    \caption{Top-k Accuracy on USPTO-LEF, $^{\dagger}$ indicate results copied from their published papers (\textcolor{blue}{additionl baselines Seq2Seq is in~\cite{schwaller2018found}, ELECTRO in~\cite{bradshaw2018electro}, and GCN in~\cite{}}), and $^{\ddagger}$ indicates results where we train and test their code. }
    \label{tab:LEF}
\end{table}
\fi

Figure~\ref{explainable} shows 
a reaction with non-linear topology  predicted by our model, where  the green box is the ground truth, which is predicted by our model correctly. Note that, our method  also predicted the  byproducts (shown in purple box) at the same time when generating the  whole predicted graph $\hat G^p$. 

 Figure~\ref{explainable} shows that our model correctly predicted the bond formation (in blue) and bond breaking (in red). This is explained by the predicted number   next to the pushing array,   indicating the predicted edge change $\hat e_{ij}$ as discussed in Equation~\ref{wwij}. Recall from Section~\ref{decodingsec} that by rounding $\hat e_{ij}$ to discrete values $\hat e^p_{ij}$, as described in Equation \ref{edgeGeneration}, we obtain the bond changes. 
 %, due to the randomness well captured by latent $z$ (see appendix, controllability of z, dynamic), prediction of a given modality (indicated by z) is highly concentrated (static), adding to the confidence of MLE of $\hat e^p_{ij}$
 
% These electron flows thus result in the bond forming and bond breaking during the reaction. 
 
%Note that,  the resulted S compound is not given as ground product molecule in the dataset, therefore draw accurate molecule with atom S may require more domain knowledge, yet in fact it do not affect our model prediction for product graph. 
%\CWC{I don't follow. Is this an incorrect prediction? Tried to rewrite...}
%\why{
It is worth noting that our model predicts the electron re-distribution around all atoms in the reactants. Hence, it infers side products. 
%}
Note that the byproduct drawn as dimethylsulfoxide (DMSO) does not appear in the ground truth record for this reaction, as the dataset only contains ``major'' reaction products. Byproducts are all speculative and predicted without any labeled training examples. %\why{
To this end, following literature, we do not evaluate the side products. 
%}
%\textcolor{brown}{why: number is the predicted edge modification $\hat e_{ij}$, due to the randomness well captured by latent $z$ (see appendix, controllability of z, dynamic), prediction of a given modality (indicated by z) is highly concentrated (static), adding to the confidence of MLE of $\hat e^p_{ij}$}


%\subsection{Performance on USPTO-LEF}
 %   \paragraph{Comparison Baselines}
    
%    \textcolor{brown}{GCN \cite{gcn} is an additional baseline for USTPO LEF by CWC. See comment %https://pubs.rsc.org/en/content/articlelanding/2019/sc/c8sc04228d#!divCitation }

\if 0
\subsection{Accuracy on the USPTO-LEF Dataset}
  %  \vspace{-2mm}
The accuracy obtained on the USPTO-LEF dataset is presented in Table~\ref{tab:LEF}. 
The performance of our method is similar to that for the USPTO-MIT dataset as presented in Table~\ref{topk}. Results here show that our method performed on par with the state-of-the-art strategies, but our method has the benefits of computational speedup and interpretability. 
\fi

%\textcolor{brown}{\txetbf{GCN} is another baseline employing graph neural networks.\cite{}}
%\textcolor{brown}{why: our inferior acc on LEF make sense from the machine learning view, since our model is a general framework, and our pseudo mechanism prediction is topology-agnostic, thus more data samples with diversity may boost our model to learn more typical transformations. On the other hand, the sequential/autoregressive counterparts rely heavily on the somehow linear data samples, which mechanism is highly consistent with the inductive bias of the algorithm design, may be confused by non-LEF segments, i.e. more complex reaction topology, and perform worse on MIT than LEF.}
   % \paragraph{\textcolor{red}{Computation Speed-up?}}

 \iffalse
\subsubsection{Latent Variable $z$ for Multi-mode Prediction}
%\textcolor{blue}{impact of $z$ ...multi-mode  reaction, electron flows heat map, disentanglement of $z$ in terms of mapping to reaction topology to reflect reaction clustering, interpretability of electron flow for failed/succeeded products...}
In this section, we show that the posterior distribution latent variable $z$   learned in our method (Equation~\ref{cvaeequ}) encodes certain reaction topology information and in-turn helps predict multi-mode reactions  

In Figure~\ref{topology}, we project the latent variable $z$ into 2 dimensions with PCA.  

Dimension reduction of latent vectors. We momentum $\mu$ of latent posterior projected to the 2-D points. The Red, Green and Blue color represent reactions in branch, parallel and single linear topology respectively. The Linear topology contains relatively low information, consistent with our intuition, while the other two common reaction topology introduce complicated modes reflected in latent vectors.

\begin{figure}[H]
        \centering
        \includegraphics[width = 0.5\linewidth]{figure/latent_topology.png}
        \caption{Dimension reduction of latent vectors. We momentum $\mu$ of latent posterior projected to the 2-D points. The Red, Green and Blue color represent reactions in branch, parallel and single linear topology respectively. The Linear topology contains relatively low information, consistent with our intuition, while the other two common reaction topology introduce complicated modes reflected in latent vectors.}  
        \label{topology}
\end{figure}

how the hidden vector controls the diversity of the resulting reactions. multi-modality problem. (through sampling the $z$ to obtain diverse reaction product molecules.)...




\begin{figure}[H]
        \centering
        \includegraphics[width = 1.0\linewidth]{figure/controlability.png}
        \caption{Sampled predictions for a non-linear topology (ring) reaction. On the left is the reactant, and on the right is the product. Our outputs are figure (a),(b), and (c), corresponding to various temperature $T$ and latent vector $z$. The smaller $z$ seems to control subtle and local transformations, while larger $z$ seems to introduce noticeable deformation in a larger range. Here the our NEFG case(a)(or (b)?, no clues from dataset, more domain knowledge required) matches the ground truth. }  
        \label{topology}
\end{figure}
\subsubsection{Visualizing the Pointers}
visualize the change of $\Delta e_{i*}$ for through heatmap...
\begin{figure}[H]
        \centering
        \includegraphics[width = 1.0\linewidth]{figure/interpretability.png}
        \caption{Example of a reaction (with branch topology) predicted by our NEFG. On the left are the molecule graphs, with figure (a),(b),(c) the input, output and ground truth respectively (need an extra bond modification illustration). On the right is the heat map of our predicted pointers for electron flow.}  
        \label{topology}
\end{figure}
    
\subsection{Transfer Learning} 
Trained with USPTO-MIT and then testing on USPTO-LEF... 
    \begin{table}[H]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
        train set/test set & MIT &LEF \\
        \hline
  %      STEREO & & & \\
       MIT  & 90.1 & 90.4\\
        LEF  & N/A & 92.0 \\
    \bottomrule
    \end{tabular}
    \caption{Single Model Top-1 Accuracy for Transfer Learning}
    \label{tab:transfer}
\end{table}

   


\subsection{Performance on USPTO-STEREO}
\begin{table}[h]
    \centering
      \begin{tabular}{lllll}
        \toprule
        \multicolumn{4}{r}{Accuracies(\%)}  \\
        \cmidrule(r){2-5}
        Model Name    & Top-1 & Top-2 & Top-3  & Top-5   \\
        \midrule
        Transformer, base & 78.1  & 84.0 & 94.6 & 95.3  \\
        MEGAN & &  & &    \\

        \hline
        \hline
        Ours & & & &   \\
        \bottomrule
        % all are decreased by 0.3%
      \end{tabular}
    \caption{Top-k Accuracy on USPTO-STEREO}
    \label{tab:stereo}
\end{table}

\subsection{Supplementary Experiments}
We evaluate our model on three datasets of organic reactions: USPTO-STEREO, USPTO-MIT, and USPTO-LEF. Each set contains less reactions than the former one and is roughly a subset of the former.

Most of the publicly available reaction datasets were derived from the patent mining work of Lowe~\citep{Lowe2012ExtractionOC}, where the chemical reactions were described using a text-based representation called SMILES.

\citet{WLN2017jin} created a subset of \citet{Lowe2012ExtractionOC}'s original set by "removing duplicate and erroneous reactions". The set contains about 480K samples.

~\citet{bradshaw2018electro} created a subset of USPTO-MIT called USPTO-LEF , which contains only linear reactions. The original subset ~\citet{bradshaw2018electro} is not publicly available yet, we recreated the subset by filtering USPTO-MIT according to the same rule.

In contrast to the MIT and LEF datasets, USPTO-STEREO underwent less filtering and the stereochemical information was kept. The set contains about 1M samples.

Table \ref{LEF} and table \ref{stereo} compares our performance with baseline methods on the benchmark datasets.

The three datasets have an interesting relationship and can provide an excellent example of transfer learning. We choose train set and test set independently from the three datasets, which yields 9 combinations, including 3 ordinary tasks and 6 transfer learning tasks. Table \ref{transfer} shows our accuracy on transfer learning between the three datasets.

\begin{table}[]
    \centering
      \begin{tabular}{lllll}
        \toprule
        \multicolumn{4}{r}{Accuracies(\%)}  \\
        \cmidrule(r){2-5}
        Model Name    & Top-1 & Top-2 & Top-3  & Top-5\\
        \midrule
        WLDN FTS & 84.0 & 89.2 & 91.1 & 92.3 \\
        Seq2Seq & 82.6 & 87.3 & 88.4 & 89.8  \\
        ELECTRO & 87.0 & 92.6 & 94.5 & 95.9  \\

        \hline
        \hline
        Ours & \textbf{88.2}& \textbf{88.2}&\textbf{88.2} &\textbf{88.2}   \\
        \bottomrule
        % all are decreased by 0.3%
      \end{tabular}
    \caption{Top-k Accuracy on USPTO-LEF}
    \label{tab:LEF}
\end{table}

\begin{table}[]
    \centering
      \begin{tabular}{lllll}
        \toprule
        \multicolumn{4}{r}{Accuracies(\%)}  \\
        \cmidrule(r){2-5}
        Model Name    & Top-1 & Top-2 & Top-3  & Top-5   \\
        \midrule
        Transformer, base & 78.1  & 84.0 & 94.6 & 95.3  \\
        MEGAN & &  & &    \\

        \hline
        \hline
        Ours & & & &   \\
        \bottomrule
        % all are decreased by 0.3%
      \end{tabular}
    \caption{Top-k Accuracy on USPTO-STEREO}
    \label{tab:stereo}
\end{table}
    
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \toprule
        train set/test set & STEREO &MIT &LEF \\
        \hline
        STEREO & & & \\
       MIT  & &90.1 & 90.4\\
        LEF  & & & 92.0 \\
    \bottomrule
    \end{tabular}
    \caption{Single Model Top-1 Accuracy for Transfer Learning}
    \label{tab:transfer}
\end{table}
\fi


==> Reaction Prediction/5-conclusion.tex <==
\section{Conclusion and Future Work}
%To the best of our knowledge, our proposed model Non-autoregressive Electron Flow Generator (NEFG) is the first non-autoregressive model for reaction prediction that achieves state-of-the-art top-1 accuracy. The key idea is to decompose edges into pairs of electrons, and edge changes into electron flows, which can then be predicted in parallel with the representation of atoms. Our model predicts chemical reactions with an order of magnitude lower inference latency, compared with the state-of-the-art autoregressive machine translation based model. The excellent performance of product prediction is consistent across multiple reaction topology, suggesting that the framework is a promising new tool for designing non-autoregressive algorithms for graph generation. 


%We contributed the  first non-autoregressive electron flow model   for reaction prediction, which captures the parallel electron movement, thus the simultaneous  bond making and breaking, in molecules in one shot. 
%We novely formulate arbitrary chemical reaction using electron flow for reaction generation.../ 
% .We formulated a novel arbitrary electron flow topology for reaction generatio
We formulated chemical reaction as a  simultaneous electron redistribution problem and  solved it with a novel  multi-pointer decoding  network. 
This results in the first  non-autoregressive electron flow model   for reaction prediction, which captures %the parallel electron movement, thus
the simultaneous  bond making and breaking in molecules in one shot. 
We empirically verified that our method achieved  superior
top-1 accuracy  and  
  at least 27  times inference speedup  over  the state-of-the-art methods. 
 %We also visually demonstrated that our method's predictions are much easier for chemists to interpret owning to predicting the electron flows (i.e., pseudo-mechanism prediction). 
 
Possessing superior predictive performance,    parallel computation, and  intuitive interpretability    makes our strategy  NERF
an appealing solution to practical learning problems involving chemical reactions. 

In the future, we will investigate the potential of  
%\textcolor{brown}{why: generalize to more
applying our framework to more complicated settings such as stereochemistry. %and add more features like 3D structures (USTPO STEREO) to atom features, the properties of latent space, especially those related to reaction class and topology; generation of arbitrary atoms instead of determined ones; cycle consistency of forward reaction and retro-synthesis.%}

==> Reaction Prediction/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

